Restart-Based Security Mechanisms for Safety-Critical Embedded Systems

Many physical plants that are controlled by embedded systems have safety requirements that need to be respected at all times - any deviations from expected behavior can result in damage to the system (often to the physical plant), the environment or even endanger human life. In recent times, malicious attacks against such systems have increased - many with the intent to cause physical damage. In this paper, we aim to decouple the safety of the plant from security of the embedded system by taking advantage of the inherent inertia in such systems. In this paper we present a system-wide restart-based framework that combines hardware and software components to (a) maintain the system within the safety region and (b) thwart potential attackers from destabilizing the system. We demonstrate the feasibility of our approach using two realistic systems - an actual 3 degree of freedom (3-DoF) helicopter and a simulated warehouse temperature control unit. Our proof-of-concept implementation is tested against multiple emulated attacks on the control units of these systems.

==> Sections/discussion.tex <==
\section{Discussion}

\subsection{Increasing the Entropy}

Despite the effectiveness of restarting and software reloading in removing the malicious components from the system, this approach does not fix the vulnerabilities in the system. In other words, those vulnerabilities that may have provided the attacker an opportunity to compromise the system. As a result, after the restart any attacker can re-launch the same attack and gain control of the system. 

To prevent system from being vulnerable to the same attack, we require the system to randomize its parameters after each restart. For a malicious activity to be successful, usually, an attacker needs a set of information about the system \eg execution trace of system to perform side-channel attack and break a cryptographic key~\cite{cite a paper} and memory address of particular functions for Return-to-libc attack~\cite{cite a paper}. Randomization introduces a noise in the execution pattern of the system within each cycle, thereby, increasing the time needed by the attacker to trigger the attack. There are a considerable body of work on various randomization techniques for security protection. Schedule Randomization~\cite{cite the paper}, address space randomization~(ASLR)~\cite{cite}, Kernel Address Space Randomization~(KASLR)~\cite{cite}, Injecting random instructions without effect on the core function~\cite{cite}.




==> Sections/framework_overview.tex <==
\section{Restart-Based Security: An Overview}
\label{subsec:res-overview}


Immediately after a reboot, if all the external interfaces have remained disabled and if the software is loaded from a read-only storage, system can be considered as uncorrupted.  




\hl{In light of this observation, restarting the system is independent of previous actions of attackers and it is guaranteed to put the system in hands of the desired uncorrupted software.} \todo[inline]{@Fardin: not very clear. please rephrase -MH}


\begin{figure}[ht]
	\begin{center}
		\includegraphics[width=0.49\textwidth]{flow}
		\caption{Sequence of the events within one restart cycle.}
		\label{fig:eventorder}
	\end{center}
\end{figure}

%With this in mind, 

The high-level overview of the proposed approach is illustrated in Fig.~\ref{fig:eventorder}).
One of the core components of our approach is to use \textit{safety controller}~(SC) that stables the system during restart\footnote{The idea of safety controller is elaborated in Section \ref{sec:background}.}.
 The key idea is that, after a reboot (while the software is still uncompromised) the time of next restart must be decided such that the following conditions remain satisfied:

\begin{itemize}
 %\ci 
 \item From current time instant until the completion of the next reboot, state will remain inside the admissible region even if the adversary is in full control; and  
 %\cii
 \item  The state of the plant after completion of the next reboot is such that the SC can stabilize the system. 
\end{itemize}


The sequence of events illustrated in Fig.~\ref{fig:eventorder}) are repeated after every restart. However, at any point of time, if state is so close to the boundary of the admissible and inadmissible states such that there is no tolerance for adversarial control~(\ie if adversary takes over can crash the in very very short time), the SC remains in charge for longer and pushes the plant further into the set of admissible states $\mathcal{S}$ (refer to Section~\ref{sec:background}) until the safety margin is large enough.  


==> Sections/resiliency.tex <==
\section{{\normalfont \textsf{ReSecure}} and Attack Resiliency}

\todo[inline]{TODO:MH $-->$ Need to rewrite this section -- MH}

Most of the existing security mechanisms protect the system from specific categories of attack and providing high security assurance requires a mixture of multiple mechanisms. Even then, there are always unknown vulnerabilities that can be exploited by an attacker to perform \emph{zero-day} attacks. On the other hand, patching the OS in embedded controllers and programmable logic controllers (PLCs) against (un)known bugs and vulnerabilities is very challenging. Due to the safety-critical nature of the applications in industrial controllers, any updates to the software needs to undergo extensive testing and verification before being deployed. 
% Some malware such as the Havex remote access trojan~\cite{symantec2014cyberespionage} infects the update installers. 
% Zero-day attacks can permanently cause the complex controller to malfunction until a manual action is taken and the vulnerability is fixed. 
% Similarly, it is very difficult, if not impossible, to claim that these compromises will be detected and be recovered from. 
\textsf{ReSecure} on the other hand, guarantees complete safety of physical unit along with some graceful degradation and restoration of functionality in the presence of any type of exploits.  



In the following, we review some examples of security threats that \textsf{ReSecure} can recover.

\subsubsection{Malicious Software}
Sophisticated adversaries can create malware that seeks to infect the external media used for transfers and updates. This opens the opportunities for possible exploits and may infect the system unknowingly to the human operator \cite{state_of_em_sec}. %Code injection attacks 
Some malicious code injections requires \textit{time}, \textit{resources} and sometime \textit{physical intervention} to spread through systems. For example, the Stuxnet worm \cite{stuxnet} was able to successfully subvert industrial control systems and infect PLCs. The worm was able to get in once an infected peripheral device was connected to the main system. After gaining access, the malware 
% fetched the attack code from a remote site and 
gradually inflicted damage to the physical plant by substituting legitimate actuation commands with infected ones \textit{over a period of time}. Flame~\cite{bencsath2012cousins} is another example of malware designed specifically for espionage that spreads through USB devices and local networks. 

Such malwares get into the system from removable drives that requires physical access and later slowly spread over the network by replicating themselves. In practice, however, it is unlikely that malicious entities can gain frequent physical access to the system after every reboot. 




% Depending on the frequency of restart (which can be determined by an approach similar to that discussed in Section \ref{subsec:restart_impact}), the malicious code may not get the opportunity to spread over the system even after successful intrusion and will be wiped out once the system reboots.

\subsubsection{Stealing Sensitive Information}
An adversary may want to track side-channel signals generated by the complex controller tasks with the intention of stealing sensitive information and secrets of the system. As a matter of fact, due to the \textit{deterministic schedules} of most RTS, an attacker can extract certain system information using signals such as timing parameters of the task~\cite{cy_side_channel}, thermal profiles \cite{thermal_profile_ccs}, secret keys \cite{side_channel_key} and cache access pattern~\cite{Wang:2007:NCD:1250662.1250723}. Such side channel attacks require the adversary to perform monitoring activities for a \textit{certain period of time to improve the accuracy} of the extracted information. 
% As an example, in order to extract the execution profile of the control tasks, the attacker may need to monitor for several hyperperiods to exactly pinpoint victim tasks \cite{cy_side_channel}. The proposed restart-based method can also be effective for such cases. This is because, by utilizing the concept of 
Restarting make it possible to prevent from \textit{stabilizing} the attacker task before it can extract a certain degree of \textit{useful} information.



% It is not inconceivable that the concept of randomization can be adopted to the proposed framework in order to make the system more resilient against attacks. 




% Let us consider the scenario in which the attacker task tries to extract the legitimate (\ie victim) task’s sensitive information (\eg a crypto key), say, using a cache side-channel attack \cite{last_level_cache}. One possible approach for the attacker would be filling some cache sets with carefully-structured data before the victim task executes. Then, the victim task runs a crypto algorithm with a given input that will use some of the cache sets. Later, the attacker task can read the cache sets and measure the latencies. Such timing information will provide hints about the victim’s cryptographic algorithm and thus aid the attacker to extract the crypto key. 



\subsubsection{Denial-of-Service (DoS) Attacks}
DoS attacks is a category of attacks where the attacker exhausts the resources of the system thereby preventing the access for the legitimate user. DoS attacks can occur in two forms; \ie system-level and network-level. In system-level attacks, attacker tries to exhaust
all the memory, consume all the processor utilization or fill all the disk spaces. These eventually prevent the real-time applications from functioning. The network-level DoS relies on sending an overwhelming influx of request to overflow the target's resources. Flood of TCP/SYN packets, overflowing the data buffer and reflective pings are examples of network DoS attacks. 

Restarting can always claim all the stale resources back and enable the system to continue operation. In the RTS context, in order to perform a system-level DoS attack, the attacker may need to monitor the execution profile for the tasks using, say, side-channel attacks and then override the task code with malicious DoS routines. Besides, the DoS routines also need some time to saturate the system resources. It is worth noting that combining all these steps to launch successful attacks requires \textit{considerable} time. 

With a correct estimation of the capabilities of the attacker (how much traffic they generate or at what rate they can exhaust system resources), the system designer can formulate the cost function for the attack and find an optimal restart time (refer to Appendix). Thus we assert that the restart-based method can be a potential solution to prevent (as well as recover) the system from many DoS attacks.


%What types of attacks we can prevent? Attacks that every time when we restart we reset all the attempts of the attacker up to that point. Like DoS

%What types of Attack we can Recover? What types of Attack we can Prevent (probably a sub-part part of attacks)?




==> Sections/statistical_analysis.tex <==
\section{Anomaly Detection using Multivariate Statistical Analysis}

\subsubsection{Building the System Profile}

Let us consider $Y^{\ell} = \lbrace y_1^\ell, y_2^\ell, \cdots, y_K^\ell \rbrace^{\mathrm{T}}$ is a vector of $K$ signals that represents the \textit{legitimate} system behavior (\eg sensor values, actuator outputs, task execution time, GPS coordinates, battery level, \etc).
Since the range of values for different signals could be different, we use Min-Max normalization technique \cite[Ch. 3]{data_mining_book} and linearly scale the range of each signal $y_j^\ell$ from $[0, 1]$ as follows:
%\begin{eqnarray}
$y_j^{\ell} = \frac{y_j^{org} - y_j^{min}}{y_j^{max} - y_j^{min}}$,
%\end{eqnarray}
where $y_j^{org}$ represents the original (\eg unscaled) value and $y_j^{max} (y_j^{min})$ denotes maximum (minimum) value of the $j$-th signal. Let us denote $Y_i^\ell$ as the $i$-th signal vector that used to generate the \textit{trace} of normal system behavior. Hence $\mathcal{Y}^\ell = \lbrace Y_1^\ell, Y_2^\ell, \cdots, Y_N^\ell \rbrace$ is the set of $N$ legitimate signals that build a training profile (\eg used as \textit{ground truth} in our verification procedure). In practice, this set of legitimate training profile can be obtained when the system is operated in controlled environment (\eg in production mode, before actual deployment). 


In this framework we propose to use Hotelling's T-square ($\rm{T}^2$ test) distance method  \cite{t2test} to detect anomalous behaviors during secure execution intervals. This multivariate statistical technique utilizes both first order (\eg mean and variance) and second order (\eg covariance matrix) statistical measures.
We use this simple statistical analysis to obtain difference between legitimate profiles and observed signals. We incorporate $\rm{T}^2$ test  because it is known to provide high accuracy \cite{ye2002multivariate,dos_multivariate_2,  dos_multivariate_1, t2_hindawi} yet low computation overhead that is particularly suitable for detecting
anomalies in the short secure execution duration.

Hotelling's $\rm{T}^2$ statistic for each legitimate training signal profile $Y_i^\ell$ is determined by the following \cite[Ch. 5]{stat_book}:
\begin{equation} \label{eq:t2_distance}
\mathbb{T}_i^\ell = \left( Y_i^\ell - \bar{Y}^\ell \right)^{\mathrm{T}} {S^\ell}^{-1} \left( Y_i^\ell - \bar{Y}^\ell \right)
\end{equation}
where $\bar{Y}^\ell = \frac{1}{N} \sum\limits_{n=1}^N Y_n^\ell$ is the mean signal vector and ${S^\ell}^{-1}$ is the $K \times K$ dimensional covariance matrix for the $N$ training profiles. Each element of $s_{i,j}^{\ell}$ in $S^\ell$ is represented by
$s_{i,j}^\ell = \frac{1}{N-1} \sum\limits_{n=1}^{N} \left( y_{i,n}^\ell - \bar{y}_i^\ell \right) \left( y_{j,n}^\ell - \bar{y}_j^\ell \right)
$ where $y_{i,j} \in \mathcal{Y}^\ell$ represents the value of $i$-th ($1 \leq i \leq K$) signal (\eg $y_i^\ell$)  for $j$-th ($1 \leq j \leq N$) trace and $\bar{y}_i^\ell$ is the mean value of signal $y_i^\ell$ over $N$ training traces. Given set of signal traces $\mathcal{Y}^\ell$ our proposed approach for generating legitimate system profile involves in the following steps:

\begin{enumerate}[\em i)]
\item Calculate the mean signal vector $\bar{Y}^\ell$, covariance matrix $S^\ell$
and obtain the $\rm{T}^2$ distance $\mathbb{T}_i^\ell$ for $\forall Y_i^\ell \in \mathcal{Y}^\ell$ using Eq. (\ref{eq:t2_distance}).
\item Calculate the mean $\mu_{\mathbb{T}}^\ell = \frac{1}{N} \sum_{n=1}^N \mathbb{T}_n^\ell$ and standard deviation $\sigma_{\mathbb{T}}^\ell = \sqrt{\frac{1}{N-1} \sum_{n=1}^N - {\left( \mathbb{T}_n^\ell -  \mu_{\mathbb{T}}^\ell \right)}^2  }$. 
\item Obtain the legitimate system profile using $\rm{T}^2$ statistics as $\mathfrak{pro}^\ell = (\bar{Y}^\ell, S^\ell \mu_{\mathbb{T}}^\ell, \sigma_{\mathbb{T}}^\ell)$.
\end{enumerate}

%the traces of signal we then calculate the mean $\mu_{\mathbb{T}}^\ell$ and standard 
%the following algorithm illustrates to generate the  


\subsubsection{Verification and Detection}

At runtime (\eg during securing execution interval) the proposed framework will perform a \textit{health check} by comparing current signal values with the stored legitimate profile $\mathfrak{pro}^\ell$. Note that the  measures of signals in a given CPS are represented by multiple random variables, and typically, the random variables representing the signals often does not follow any particular distribution. However, if the training signal vectors $(\eg  Y_i^\ell)$ are independent and the number of training samples are sufficiently large (\eg $N > 30$), according to the central limit theorem \cite[Ch. 5]{stat_book} the $\rm{T}^2$ distance follows approximately a
normal distribution regardless of the distribution of individual signals $y_i^\ell$ ($1 \leq i \leq K$) \cite{ye2002multivariate, dos_multivariate_1, dos_multivariate_2}. Since we are interested in detection deviations from legitimate profile, we select $\mu_{\mathbb{T}}^\ell \pm \lambda \sigma_{\mathbb{T}}^\ell$ 
as an anomaly detection threshold, that is, if the $\rm{T}^2$ distance for
 an observation %$i$ (referred to as $\mathbb{T}_i^o$) 
 (\ie $\mathbb{T}^o$)
 is \textit{not} within the range $[\mu_{\mathbb{T}}^\ell - \lambda \sigma_{\mathbb{T}}^\ell, \mu_{\mathbb{T}}^\ell + \lambda \sigma_{\mathbb{T}}^\ell]$ we mark the set of signals as anomaly, where $\lambda$ represents the confidence interval, usually ranging from $1$ to $3$ for confidence
levels ranging from 68\% to 99.7\% \cite{dos_multivariate_2, dos_multivariate_1}. 

Given the legitimate profile $\mathfrak{p}^\ell$, when the set of (normalized) signal vector $Y^{o} = \lbrace y_1^o, y_2^o, \cdots, y_K^o \rbrace^{\mathrm{T}}$ is accessed at the secure execution interval, we can therefore classify the signals (\eg normal or anomalous) based on the aforesaid detection threshold. The overall detection procedure is summarized in Algorithm \ref{alg:t2_int_detect}.


\begin{algorithm}[t]

\newcommand{\algorithmicbreak}{\textbf{break}}
\newcommand{\BREAK}{\STATE \algorithmicbreak}
\renewcommand\algorithmiccomment[1]{%
 {\it /* {#1} */} %
}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
    \renewcommand{\algorithmicensure}{\textbf{Output:}}

\begin{algorithmic}[1]
\begin{footnotesize}
\REQUIRE The legitimate profile $\mathfrak{pro}^\ell = (\bar{Y}^\ell, S^\ell \mu_{\mathbb{T}}^\ell, \sigma_{\mathbb{T}}^\ell)$, confidence level of detection $\lambda$ and the set of normalized observation signals $Y^{o} = \lbrace y_1^o, y_2^o, \cdots, y_K^o \rbrace^{\mathrm{T}}$
    \ENSURE The boolean variable $\mathtt{isAnomalous}$ indicates whether the observation signals $Y^{o}$ are \textit{normal} or \textit{anomalous}
\vspace{0.2em}
%\vspace*{-0.5em}

\STATE $\mathtt{isAnomalous} := \textbf{true}$ ~~\COMMENT{initialize the boolean variable}

\STATE Calculate $\rm{T}^2$ distance for observed signals as follows:
$$\mathbb{T}^o =  \left( Y^o - \bar{Y}^\ell \right)^{\mathrm{T}} {S^\ell}^{-1} \left( Y^o - \bar{Y}^\ell \right)$$


\IF {$\mathbb{T}_i^o \in [\mu_{\mathbb{T}}^\ell - \lambda \sigma_{\mathbb{T}}^\ell, \mu_{\mathbb{T}}^\ell + \lambda \sigma_{\mathbb{T}}^\ell]$}
\STATE \COMMENT{within threshold range, normal behavior}
\STATE $\mathtt{isAnomalous} := \textbf{false}$  
				\ENDIF
        
                
       \RETURN  $\mathtt{isAnomalous}$

\end{footnotesize}

\end{algorithmic}
\caption{Intrusion detection based on $\rm{T}^2$ statistics}
\label{alg:t2_int_detect}
\end{algorithm}






==> for arXiv/Sections/adversary.tex <==
\section{System and Adversary Model}
\label{sec:model}
%\subsection{Safety-Critical Embedded CPS}

\subsection{System Model}

The type of system that we consider in this work is an embedded control system that drives the physical plant. Examples of such systems include heating, ventilation and watering systems, smart home appliances, drone control systems, automotive engine controllers, process controllers, \etc  These systems usually provide an interface to interact with user or other physical systems. These interfaces may be utilized for transmitting the state and sensors values or receiving new set points and operation plans. In some cases, embedded platforms also provide debugging interfaces that can be used for diagnosing errors during operation or the development cycle. Furthermore, the physical plant has \textit{safety requirements} that need to be respected at \textit{all} times. Failure to satisfy the safety requirements may damage the physical components or surrounding environment. As an example, a helicopter/UAV may destabilized (or damaged) if its wings touches the ground or other objects.

%in a food transport truck, the temperature must never drop below or above an specified range or the food will be spoiled. 

%\subsection{Adversarial Capabilities and Assumptions}

\subsection{Adversary Model}

Embedded CPS face threats in various forms depending on the system and the goals of the attacker. For instance, adversaries may insert, eavesdrop on or modify messages exchanged by system components. Besides, attackers may manipulate the processing of sensor inputs and actuator commands, could try to modify the control flow of the system as well as extract sensitive information through side-channels. In this paper we make the following assumptions about the system and capabilities of the adversary:


\begin{enumerate}[\it i\normalfont )]
	
	\item \textit{Software image integrity:} We assume that the original image of the system software~(real-time operating system~(RTOS), control applications and other components) does not contain malicious components. These components, however, may contain bugs or security vulnerabilities that could be exploited to initiate attacks.
	
	\item \textit{Read-only memory unit}: We assume that the original image of the system software is stored on a read-only memory unit (\ie E$^2$PROM). This content is unmodifiable at runtime by adversary or other entities.

	\item \textit{Integrity of Root of Trust (RoT)}: As mentioned earlier, RoT is an isolated hardware module responsible for issuing a restart signal %to the restart pin of the platform 
    at designated times. It is designed to be directly accessible \textit{only} during an internal that we call the SEI~(refer to Section~\ref{sec:RoTDesign}). Hence, we consider that attackers can not compromise it to prevent the system from restarting. 	
	
	\item \textit{Sensor and actuator integrity}: We assume that the adversary does not have physical access to the sensors and actuators. Hence, values reported by sensors are correct and commands sent to the actuators are executed accordingly. However, an attacker may corrupt and replace sensor measurements or actuator commands inside the applications, on the network or underlying OS.
	
	\item \textit{External attacks}: Attackers require an external interface such as the network, serial port or debugging interface to launch the attacks. As long as all such interfaces remain disabled, applications running on the system are assumed to be trusted. 

	\item \textit{Integrity violation}: We assume that once the external interfaces are activated, the adversary can compromise the software components\footnote{We are not concerned with exact method used by attackers to get into the system.} on the embedded system including the RTOS as well as the real-time/control applications. 

%	For example, an adversary may insert a malicious task that respects the real-time guarantees of the system to avoid immediate detection, compromise one or more existing real-time tasks and/or may override parts of the underlying RTOS itself that may eventually threaten overall safety of the system.	
	
\end{enumerate}


%Under the above assumptions,
% Given the aforementioned  adversarial capabilities implementing the proposed restart-based mechanism provides \textit{guaranteed} protection of the the physical system under malicious activities (\eg those targets to damage the physical plant).

% for the physical system from attacks whose target is to damage the physical plant. 
%In other words, 
%In summary, our proposed method intruders cannot take the system outside of the safety region under any circumstance.
%\todo[inline]{Say things we can protect  with forward pointers to the future sections that does that. Mention the attacks that we do not protect}
%\todo[inline]{Mention the worst case attacks and how it can be handled}
%\todo[inline]{And mention that it is not our concern how the attacker gets into the system}
%Moreover, 
%Besides, 

Our approach also improves system security against forms of attack that have intentions other than damaging the physical plant. The following are some instances of such attacks \cite{cy_side_channel,mhasan_resecure16}: \ci \textit{Information leakage through side-channels}: The adversary may aim to learn important information through side or covert-channel attacks by simply lodging themselves in the system and extracting sensitive information. \cii \textit{System-level Denial of Service (DoS)}: The attacker may intrude into the real-time system and exhaust \textit{system-level} resources such as CPU, disk, memory, restricting safety-critical control tasks from necessary resources, \etc~ 
%An advanced attacker may capture I/O or network ports and perform \textit{network-level} attacks to tamper with the confidentiality and integrity of the system. 
\ciii \textit{Control performance degradation}:
An attacker may focus on reducing the control performance and consequently reducing the progress of the system towards the mission goal by tampering with actuators/sensors and/or preventing the control processes from proper execution.

Our approach does not mitigate network attacks such as man-in-the-middle or DoS attacks that restrict network access. Also, the safety guarantees of the physical plant do not hold if the system is susceptible to sensor jamming attacks (\eg GPS jamming, electromagnetic interference on sensors \etc). 

%
%\begin{enumerate}[\it i\normalfont )]
%
%\item \textit{Control performance degradation}: The attacker may avoid trying to cause an immediate damage and instead focus on reducing the control performance of the system by changing the values of the actuators and system system set points.
%
%\item \textit{Denial of Service (DoS)}: The attacker may take control of the real-time task(s) in the controller and perform \textit{system-level} resource (\eg CPU, disk, memory, \etc) exhaustion.  In addition, an advanced attacker may capture I/O or network ports and perform \textit{network-level} attacks to tamper with the confidentiality and integrity (\viz safety) of the system.
%
%\item \textit{Information leakage through side-channels}:
%The adversary may also aim to learn important information by side or covert-channel attacks by simply lodging themselves in the system and extracting sensitive information. For example, the intruder may utilize side-channels to monitor the system behavior and infer certain degree of system information (\eg hardware/software architecture, and \etc) that eventually leads to the attacker actively taking control, manipulating and/or crashing the system. 
%\end{enumerate}





==> for arXiv/Sections/background.tex <==
%\section{Background on Safety Controller~(SC)}
\section{Background on Safety Controller}
\label{sec:background}

As we explain in Section \ref{sec:details}, a core component of our approach is the \textit{safety controller~(SC)}. Since the properties of the SC is essential for our approach, we now introduce this concept and illustrate a method to construct the SC. In the next section, we will use these concepts to establish the restart-based protection. For ease of understanding we first present some useful definitions before describing the details of SC design.


\begin{definition}[Admissible and Inadmissible States]
States that do not violate any of the operational constraints are referred to as \textit{admissible states} and denoted by $\mathcal{S}$. Likewise those that violate the constraints are referred to as \textit{inadmissible states} and denoted by $\mathcal{S}'$.
\end{definition}



%From this definition, we can then define the set of states that are recoverable for a particular control strategy, assumed to be a given safety controller in the Simplex architecture.

%\textbf{Definition}: 

\begin{definition}[Recoverable States]
\textit{Recoverable states}, a subset of the admissible states, such that if any given SC starts operations from one of those states, all future states will remain admissible. The set of recoverable states is denoted by $\mathcal{R}$.
\end{definition}


%\cite{sha1998dependable,Sha01usingsimplicity,sha1996evolving,crenshaw2007simplex},

%From the above definitions, the set of admissible states is derived from safety constraints of the system. 

To implement our restart-based protection approach, one must construct an SC for the system and find its associated $\mathcal{R}$. For this, we provide a brief overview of constructing a SC introduced in earlier literature~\cite{seto1999case}\footnote{Any other design method for constructing an SC and the corresponding recoverable region~$\mathcal{R}$ with the above properties can be utilized for the purpose of the framework introduced in this paper.}. %In the approach of literature~\cite{seto1999case}, 
%One approach to construct a safety controller is proposed in~\cite{seto1999case}. We provide a brief overview of this method in this section. 
%Notice
%It is worth mentioning that,
According to this approach, 
the SC is designed by approximating the system with linear dynamics in the form of $\dot{x} = Ax + Bu$, for state vector $x$ and input vector $u$. In addition
%approach, 
\emph{the safety constraints of the physical system are expressed as linear
constraints} in the form of $H \cdot x \leq h$ where $H$ and $h$ are constant matrix and vector. Consequently, the set of admissible states are $\mathcal{S} = \{x: H \cdot x \leq h \}$.


Safety constraints, along with the linear dynamics for the system are the inputs to a convex optimization problem. %\footnote{For details, please refer to~\cite{seto1999case}.} 
%that 
These parameters
produce both linear proportional controller gains $K$ as well as a positive-definite matrix $P$. The resulting linear-state feedback controller, $u = Kx$, yields closed-loop dynamics in the form of $\dot{x} = (A + BK)x$. Given a state $x$, when the input $u = Kx$ is used, the $P$ matrix defines a Lyapunov potential function $(x^TPx)$ with a negative-definite derivative. As a result, for the states where $x^TPx < 1$, the stability of the linear system is guaranteed using Lyapunov's
direct or indirect methods.
%\footnote{For details of this analysis we refer the readers to literature~\cite{seto1999case}.}. 
%Furthermore, the matrix $P$ defines an ellipsoid in the state space where all safety constraints are satisfied when $x^TPx < 1$. 
It follows that the states which satisfy $x^TPx < 1$ are a subset of the safety region. As long as the system's state is inside $x^TPx < 1$ and the $u = Kx$ is the controller, the physical plant will be driven toward the equilibrium point, \ie $x^TPx = 0$. Since the potential function is strictly decreasing over time, any trajectory starting inside the region $x^TPx < 1$ will remain there for an unbounded time window. %Therefore 
As a result
no inadmissible states will be reached. %In the light of these results, 
Hence, the 
linear-state feedback controller $u = Kx$ is the SC and $\mathcal{R} = \{ x : x^TPx < 1\}$ is the recoverable region. Designing SC in such way ensures that the physical system would remain always safe \cite{Sha01usingsimplicity}.



%
%Restarting a computational unit in charge of controlling a physical system is a challenging problem. The restarting mechanism need to provide guarantees that  during the restart the safety-requirements of the physical system remain satisfied. There are two main works~\cite{fardin2016reset} and~\cite{abdi2017application}, that are specifically designed to enable restarting safety-critical embedded system. While, the main goal of these architectures is to provide fault-tolerance and fault-recovery, they can also be used to perform safe restarting to improve security. 
%
%%
%%\subsection{Restarting Using a Back Up Controller}
%%
%%The architecture proposed in~\cite{fardin2016reset}, is a variation of Simplex Architecture~\cite{sha1998dependable, Sha01usingsimplicity, sha1996evolving}. This design consists of two control units. First, a main control unit, also known as Complex Control unit, that may contain logical or implementation bugs. Second, a second back up controller unit called safety unit which contains a safety controller and a decision module. Components of the safety unit are logically correct and verified~(bug-free). The safety controller is able to recover and stabilize the system as long as the state is inside a recovery region. Hence, in runtime, if the state of the system is close to the boundary of the recovery region, the decision module switches the control the safety controller. As a result, misbehaviors in the complex unit~(OS or applications) does not affect the safety of the physical system.
%%
%%
%%\begin{figure}[ht]
%% \begin{center}
%%   \includegraphics[width=0.49\textwidth]{architecture-resecure}
%%   \caption{Logical view of Simplex architecture using extra hardware.}
%%   \label{fig::simplex}
%% \end{center}
%%\end{figure}
%
%\subsection{Restartable Controller Design}
%
%A recent work in~\cite{abdi2017application} explains the procedure to design a controller that enables the entire computing system to be safely restarted at runtime. This controller is called \emph{base controller} and has the following property. Base Controller keeps the system inside a subset of safety region, only by updating the actuator input at least once after every system restart. In other words, after a restart, system can restart immediately after only one command is applied to the actuators. During a restart, a fresh image of all the software~(middleware, RTOS, and applications) is loaded from a read-only storage which recovers the system into an operational state. 
%
%Having only Base Controller, allows the system to remain safe and tolerate software faults and recover from them~(by performing  a restart). However, the system does not make any progress towards its mission goal. To address this issue, Base Controller is complemented with a Mission controller and a Decision Module. MC is a high-performance, complex controller that drives the system towards the mission setpoints. To maximize the progress towards the mission goals, in every control cycle, Decision Module checks the Mission Controller command. If it satisfies the safety requirements, it allows the Mission Controller command to be sent to the actuators. Otherwise, Base Controller command is applied to the system. By doing so, Mission Controller drives the system for as long as possible, And, whenever it is not possible, Base Controller takes the control. 
%
%
%%In the proposed design, the only components that need to be verified for correct functionality are BC, DM and Flushing Task. Any faults in the system software~(System-Level or Application-Level) that results in a fail-silent failure~(also known as fail-stop) of these two components leads to WD triggering a system-wide restart and recovery. However, our design does not protect the system from faults that alter the logic of BC or DM at execution time. In summary, this design enables the system to provide formal safety guarantees by verifying only the correctness of BC, DM and Flushing Task instead of entire MC, RTOS, and middleware. 
%
%%
%%
%%\begin{figure}[ht]
%% \begin{center}
%% \includegraphics[width=0.49\textwidth]{architecture-ICCPS}
%%   \caption{The logical view of the proposed design.}
%%   \label{fig:architecture}
%% \end{center}
%%\end{figure}





==> for arXiv/Sections/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
	In this paper, we aim to decouple the \textit{safety} requirements of the physical plant from 
the \textit{security} properties. %. of the embedded system. 
Because of inertia, pushing 
%an embedded system that controls 
a physical plant from a given (potentially safe) state to an unsafe state --
even with complete adversarial control -- is not instantaneous and often takes 
finite (even considerable) time. We leverage
this property to calculate a \textit{safe operational window} and combine it with the effectiveness of {\em system-wide
	restarts} to decrease the efficacy of malicious actors.
%In this paper we present a 
%The proposed restart-based framework that combines hardware  and software components to \ca maintain the system within the safety region and \cb thwart potential attackers from destabilizing the system.
Designers of such safety-critical systems can now evaluate
the necessary trade-offs between control system performance and
increased security guarantees -- thus improving the overall design of embedded CPS in the future.


==> for arXiv/Sections/discussion.tex <==
\section{Discussion}

\subsection{Increasing the Entropy}

Despite the effectiveness of restarting and software reloading in removing the malicious components from the system, this approach does not fix the vulnerabilities in the system. In other words, those vulnerabilities that may have provided the attacker an opportunity to compromise the system. As a result, after the restart any attacker can re-launch the same attack and gain control of the system. 

To prevent system from being vulnerable to the same attack, we require the system to randomize its parameters after each restart. For a malicious activity to be successful, usually, an attacker needs a set of information about the system \eg execution trace of system to perform side-channel attack and break a cryptographic key~\cite{cite a paper} and memory address of particular functions for Return-to-libc attack~\cite{cite a paper}. Randomization introduces a noise in the execution pattern of the system within each cycle, thereby, increasing the time needed by the attacker to trigger the attack. There are a considerable body of work on various randomization techniques for security protection. Schedule Randomization~\cite{cite the paper}, address space randomization~(ASLR)~\cite{cite}, Kernel Address Space Randomization~(KASLR)~\cite{cite}, Injecting random instructions without effect on the core function~\cite{cite}.




==> for arXiv/Sections/evaluation.tex <==
\section{Evaluation}
\label{sec:evaluation}

We now evaluate various aspects of restart-based protection approach using a combination of simulation-based and an actual implementation. To evaluate practicality, we compare the safe restart times for two target systems, a 3-degree of freedom helicopter~\cite{3dof} and a warehouse temperature system~\cite{trapnes2013optimal}. The former is a very unstable system with fast-moving dynamics and the latter is a relatively stable system with slower dynamics. In addition, we have implemented a controller on a commercial-off-the-shelf~(COTS) ZedBoard~\cite{zboarddatasheet} embedded platform for a realistic 3DOF helicopter. We perform platform attacks on the embedded system and empirically demonstrate that the helicopter remains safe and recovers from the attacks.


\subsection{Physical Systems Under Evaluation}


\subsubsection{3-Degree of Freedom Helicopter:} 3DOF helicopter~(displayed in figure~\ref{fig:3dof}) is a simplified helicopter model, ideally suited to test intermediate to advanced control concepts and theories relevant to real-world applications of flight dynamics and control in the tandem rotor helicopters, or any device with similar dynamics~\cite{3dofhelicopter}. It is equipped with two motors that can generate force in the upward and downward direction, according to the given actuation voltage. It also has three sensors to measure elevation, pitch and travel angle as shown in Figure~\ref{fig:3dof}. We use the linear model of this system obtained from the manufacturer manual~\cite{3dofhelicopter} for constructing the safety controller and calculating the reachable set in run-time. Due to the lack of space, the details of the model are included in our technical report~\cite{githubrepoemsoft}.




For the 3DOF helicopter, the safety region is defined in such a way that the helicopter fans do not hit the surface underneath, as shown in Figure~\ref{fig:3dof}. The linear inequalities describing the safety region are provided are $-\epsilon + |\rho| \leq 0.3$ and $|\rho| \leq \pi/4$. Here, variables $\epsilon$, $\rho$, and $\lambda$ are the elevation, pitch, and travel angles of the helicopter. Limitations on the motor voltages of the helicopter are $|v_l| \leq 1.1$ and $|v_r| \leq 1.1$ where $v_l$ and $v_r$ are the voltage for controlling left and right motors.



%
%\begin{equation}
%\label{eq:safetyQuanser}
%\left[
%\begin{array}{cccccc}
%-1 & -0.33 & 0 & 0 & 0 & 0 \\
%-1 & 0.33 & 0 & 0 & 0 & 0 \\
%%% 1 & 0 & 0 & 0 & 0 & 0 \\
%%% -1 & 0 & 0 & 0 & 0 & 0 \\
% 0 & 1 & 0 & 0 & 0 & 0 \\
% 0 & -1 & 0 & 0 & 0 & 0 \\
%%0 & 0 & 0 & 1 & 0 & 0 \\
%%0 & 0 & 0 & -1 & 0 & 0 \\
%%0 & 0 & 0 & 0 & 1 & 0 \\
%%0 & 0 & 0 & 0 & -1 & 0 \\
%\end{array}
%\right]
%%\left[
%%\begin{array}{c}
%%\epsilon \\
%%\rho\\ 
%%\lambda\\
%%\dot{\epsilon}\\
%%\dot{\rho}\\
%%\dot{\lambda}\\
%%\end{array}
%%\right]
%x
%\leq
%\left[
%\begin{array}{c}
%0.3\\
%0.3\\
%%% 1\\
%%% 1\\
% \pi/4\\
% \pi/4\\
%%0.4\\
%%0.4\\
%%1.5\\
%%1.5\\
%\end{array}
%\right]
%\end{equation}



\subsubsection{Warehouse Temperature System:}
This system consists of a warehouse room 
with a direct conditioner system~(heater and cooler) to the room and another conditioner in the floor. The safety goal for this system is to keep the temperature of the room within the range of $[20^{\circ}C,30^{\circ}C]$. This system and its model are obtained from the work in~\cite{trapnes2013optimal}. Equations~\ref{eq:heatermodel1} and~\ref{eq:heatermodel2} describe the heat transfer between the heater and floor, floor and the room, and room and outside temperature. The model assumes constant mass and volume of air and heat transfer only through conduction.



\begin{equation}
\dot{T}_F = -\frac{U_{F/R} A_{F/R}}{m_FCp_F}(T_F-T_R) + \frac{u_{H/F}}{m_FCp_F}
\label{eq:heatermodel1}
\end{equation}
\begin{equation}
\dot{T}_R = -\frac{U_{R/O} A_{R/O}}{m_RCp_R}(T_R-T_O) + \frac{U_{F/R}A_{F/R}}{m_RCp_R}(T_F-T_R) + \frac{u_{H/R}}{m_RCp_R}
\label{eq:heatermodel2}
\end{equation}
Here, $T_F$, $T_R$, and $T_O$ are temperature of the floor, room and outside. $m_F$ and $m_R$ are the mass of floor and the air in the room. $u_{H/F}$ is the heat from the floor heater to the floor and $u_{H/R}$ is the heat from the room heater to the room both of which are controlled by the controller. $Cp_F$ and $Cp_R$ are the specific heat capacity of floor~(in this case concrete) and air. $U_{F/R}$ and $U_{R/O}$ represent the overall heat transfer coefficient between the floor and room, and room and outside. 


For this experiment, the walls are assumed to consist of three layers; the inner and outer wall are made of oak, and isolated with rock wool in the middle. The floor is assumed to be quadratic and consists of wood and concrete. The parameters used are as following\footnote{For the details of calculation of $U_{F/R}$ and $U_{R/O}$ and the values of the parameters refer to Chapter 2 and 3 of~\cite{trapnes2013optimal}.}: $U_{R/O} = 539.61J/hm^2K$, $U_{F/R} = 49920 J/hm^2K$ , $m_R = 69.96kg$, $m_F = 6000kg$, floor area $A_{F/R} = 25 m^2$, wall and ceiling area $A_{R/O} = 48 m^2$, thickness of rock wool, oak and concrete in the wall and floor respectively $0.25m$, $0.15m$ and $0.1m$. Maximum heat generation capacity of the room and floor conditioner is respectively $800J/s$ and $115J/s$. And, maximum cooling capacity of the room and the floor cooler is $-800J/s$ and $-115J/s$.


\subsection{Safe Restart Time for the Physical Systems}

\label{sec:restarttimeeval}

%Our goal in this section is to evaluate the practicality of using our technique in different physical systems. As discussed before, the intuitive definition of safe operation time~(which we use to set the next restart time) is the shortest time that an attacker needs to take the system to an unsafe state. 


As discussed in the previous sections, after each system reboot the time of the next restart of the embedded system needs to be computed. The main factor that impacts the safe restart time is the proximity of the current state of the plant to the boundaries of the inadmissible states. In this section, we demonstrate this point on two physical systems with fast and slow dynamics; 3DOF helicopter and warehouse temperature system.


%is an unstable system with a fairly small safety margin. On the other side, warehouse temperature system has slow dynamics and the pace of the temperature change even with maximum heating or cooling allows a large safety margin. 

In figures~\ref{fig:exp1} and~\ref{fig:exp2}, the calculated safe restart times are plotted for the two systems under investigation. In these figures, the red region represents the inadmissible states and the plant must never reach to those states. If the plant is in a state that is marked green, it is still undamaged. However, at some future time it will reach an inadmissible state and the safety controller may not be able to prevent it. This is because physical actuators have a limited range and the maximum capacity of the actuators is not enough to cancel the momentum and prevent the plant from reaching the unsafe states. And the gray/black area is the region in which a value for the safe restart time of the system can be computed. In this region, the darkness of the color indicates the value of calculated restart time if the plant is in that state. The black points indicate the maximum time and the white points are an indicator of zero time. 


\begin{figure}[ht]
	\begin{center}
		\centering 
		\subfigure[Projection of the state space into the plane $\dot{\epsilon} = 0$, $\dot{\rho} = 0$, $\lambda = 0$, and $\dot{\lambda} = 0.3\text{Radian}/s$]
			{\label{fig:exp11}\includegraphics[width=0.22\textwidth]{Figures/exps/e11}}
		\hfil
		\subfigure[Projection of the state space into the plane  $\dot{\epsilon} = -0.3\text{Radian}/s$, $\dot{\rho} = 0$, $\lambda = 0$, and $\dot{\lambda} = 0.3\text{Radian}/s$]
		{\label{fig:exp12}\includegraphics[width=0.22\textwidth]{Figures/exps/e12}}
		\caption{Calculated safe restarting time for the 3DOF helicopter system from various states. Darkest black points represent a possible restart time of 1.23 seconds.}
		\label{fig:exp1}
	\end{center}
\end{figure}

In Figure~\ref{fig:exp1}, for 3DOF helicopter, the maximum calculated safe restart time~(\ie the darkest points in the gray region) is $1.23$ seconds. As seen in the Figure, restart time is maximum in the center where it is farthest away from the boundaries of unsafe states. In Figure~\ref{fig:exp12}, the angular elevation speed of the helicopter is $\dot{\epsilon} = -0.3\text{Radian}/s$. This indicates that the helicopter is heading towards the surface with the rate of 0.3 Radian per second. As a result, the plant cannot be stabilized from the lower elevations levels~(\ie the green region). Moreover, values of the safe restart times are smaller in Figure~\ref{fig:exp12} compared to the Figure~\ref{fig:exp11}. Because, crashing the 3DOF helicopter with the initial downward speed requires less time than the case without any downward angular velocity.


\begin{figure}[ht]
	\begin{center}
		\centering 
		\subfigure[Projection of states to $T_F = 25ºC$]
		{\label{fig:exp21}\includegraphics[width=0.22\textwidth]{Figures/exps/e21}}
		\subfigure[Projection of states to $T_F = 29ºC$]
		{\label{fig:exp22}\includegraphics[width=0.22\textwidth]{Figures/exps/e22}}
		\caption{Safe restarting times calculated for the embedded controller system of warehouse temperature.}
		\label{fig:exp2}
	\end{center}
\end{figure}

Figures~\ref{fig:exp21} and~\ref{fig:exp21}, plot the calculated safe restart times for the warehouse temperature system. For this system, when the outside temperature is too high or too low, the attacker requires less time to take the temperature beyond or bellow the safety range. One major difference of this system with the 3DOF helicopter is that due to the slower dynamics, the safe restart times have values up to $6235s$~(close to one hour and forty minutes). In the warehouse system, the rate of the change of the temperature even when the heater/coolers run at their maximum capacity is slow and hence, attacker needs more time to take the system to unsafe states.

%Note that for a given system, values calculated safe restart times is impacted by two main factors: \ci the current state of the plant \cii actuator operation range. If system is closer to the boundaries of the unsafe states, it can get damaged in shorter time. However, the impact of the actuator limits are more complicated. The more powerful actuator means that the attacker can drive the system towards instability faster but at the same time, the safety controller has more power to stabilize the system. 


If above systems are restarted at times smaller than the calculated safe restart windows, the physical plant is guaranteed to remain safe under an attacker who gains full control immediately after SEI ends. Achieving this goal is very reasonable for systems such as the warehouse temperature control and many other similar systems with applications in Internet of Things~(IoT), city infrastructure, and \etc. For systems with faster and more unstable dynamics such as the helicopter, the calculated restart times might become very short. The fast restart rate, even though theoretically possible, in practice may create implementation challenges. For instance, initializing a connection with the remote user over Internet may require more time than the calculated safe restart time. For our particular 3DOF controller implementation~(Section~\ref{sec:implementation}), we use serial port for communication which has a very small initialization overhead. Despite short restart times, we demonstrate that the system remains stable and functional.

%If the implementation challenges do not allow such short restart times, from the analysis of Section~\ref{sec:probability}, depending on the probability function of attacks for the system, the security of the system may improve with fixed periodic restarts.





\subsection{Restarting and  Embedded System Availability}
During the restart, embedded system is unavailable and actuators keep executing the last command that was received before the restart occurred. Results of Theorem~\ref{thm:safety} guarantees that such unavailability does not compromise safety and stability of the physical plant. However, low availability may slow down the progress of the system towards its control mission. In this section, we measure the average percent of the time that the embedded system is available when restart-based protection is implemented. The approach is as follows. 


Availability of the controller is the ratio of the time that the main controller is running~(not rebooting and not in SEI) to the whole operation time of the system. In every restart cycle, availability is $ (\delta_r)/(\delta_r + T_s + T_r)$ where $\delta_r$ is the safe restart time~(main controller is active during $\delta_r$), $T_s$ is the length of SEI, and $T_r$ is the reboot time of the embedded platform. Value of $\delta_r$ is not fixed and changes according to the state of the plant. To measure availability, we divide the state space into three sub-regions based on how often the physical plant is expected to operate in those regions.  The availability values computed for the states in the most common region are assigned a weight of \emph{1}, second most common region a weight of \emph{0.5} and the least common region a weight of \emph{0.3}. We calculated the expected availability of the controller for all the states in the operational range of the system.  At the end, the weighted average of the availability was calculated according to the aforementioned weights. For the value of the $T_r$, we used $390ms$ for the reboot time of the 3DOF embedded controller~(Measured for the ZedBoard~\cite{zboarddatasheet} used in the implementation of the controller in next section) and $10s$ 
for reboot time of the temperature controller embedded system~(we assumed platform with embedded Linux OS). The ranges for the regions and obtained availability results are presented in Table~\ref{table:availability}. 

From these results, the impact of our approach on the temperature control system is negligible. However, there is a considerable impact on the availability of the helicopter controller due to frequent restarts. Notice that, the helicopter system is among the most unstable systems and therefore, one of the most challenging ones to provide \emph{guaranteed} protection. As a result, the calculated results for the helicopter system can be considered as an approximated upper bound on the impact of our approach on controller availability among all the systems.In the next section, we use a realistic 3DOF helicopter and demonstrate that, despite the reduced the availability, the plant remains safe and stable and makes progress. 

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
%\begin{table}[hb]
%	\centering
%
%	\label{table:availability}
%	\begin{tabular}{c|c|c|}
%		\cline{2-3}
%		& \cellcolor[HTML]{C0C0C0}\begin{tabular}[c]{@{}c@{}}Regions (From most\\ common to least Common)\end{tabular} & \cellcolor[HTML]{C0C0C0}Avail. \\ \hline
%		\multicolumn{1}{|c|}{\cellcolor[HTML]{C0C0C0}}                                                                                         & 15\textless $T_O$ \textless 40                                                                                                           &                                      \\ \cline{2-2}
%		\multicolumn{1}{|c|}{\cellcolor[HTML]{C0C0C0}}                                                                                         & 0\textless $T_O$ \textless 15 or 40 \textless $T_O$ \textless 60                                                                                                           &                                      \\ \cline{2-2}
%		\multicolumn{1}{|c|}{\multirow{-3}{*}{\cellcolor[HTML]{C0C0C0}\begin{tabular}[c]{@{}c@{}}Temperature\\ Control\\ System\end{tabular}}} & $T_O$ \textless 0 or 60 \textless $T_O$                                                                                                           & \multirow{-3}{*}{\%99.9}             \\ \hline
%		\multicolumn{1}{|c|}{\cellcolor[HTML]{C0C0C0}}                                                                                         & $-\epsilon + |\rho| <$  0.1 \& $\epsilon < 0.2$ \& $|\rho| < \pi/8 $                                                                                                           &                                      \\ \cline{2-2}
%		\multicolumn{1}{|c|}{\cellcolor[HTML]{C0C0C0}}                                                                                         & 0.2$< -\epsilon + |\rho| <$  0.1 \& $0.2<\epsilon < 0.3$                                                                                                            &                                      \\
%		
%		\multicolumn{1}{|c|}{\cellcolor[HTML]{C0C0C0}}                                                                                         &
%		
%		 \multicolumn{1}{c|}{\& $\pi/8 < |\rho| < \pi/6$}                                                                                        &                                      \\ \cline{2-2}
%		\multicolumn{1}{|c|}{\cellcolor[HTML]{C0C0C0}}                                                                                         & $ -\epsilon + |\rho| <$  0.2 \& $0.3<\epsilon$ \& $\pi/6 < |\rho| $                                                                                                            &                                      \\
%		\multicolumn{1}{|c|}{\multirow{-5}{*}{\cellcolor[HTML]{C0C0C0}\begin{tabular}[c]{@{}c@{}}3DOF\\  Helicopter\end{tabular}}}             & \multicolumn{1}{l|}{}                                                                                        & \multirow{-5}{*}{\%64.3}             \\ \hline
%	\end{tabular}
%	\caption{Weighted average availability of the embedded system.}
%\end{table}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}

\begin{table}[]
	\centering
	\begin{tabular}{c|c|c|}
		\cline{2-3}
		& \cellcolor[HTML]{C0C0C0}\begin{tabular}[c]{@{}c@{}}Regions (From most\\ common to least Common)\end{tabular} & \cellcolor[HTML]{C0C0C0}Avail. \\ \hline
		\multicolumn{1}{|c|}{\cellcolor[HTML]{C0C0C0}}                                                                                         & 15\textless $T_O$ \textless 40                                                                                                            &                                \\ \cline{2-2}
		\multicolumn{1}{|c|}{\cellcolor[HTML]{C0C0C0}}                                                                                         & 0\textless $T_O$ \textless 15 or 40 \textless $T_O$ \textless 60                                                                                                           &                                \\ \cline{2-2}
		\multicolumn{1}{|c|}{\multirow{-3}{*}{\cellcolor[HTML]{C0C0C0}\begin{tabular}[c]{@{}c@{}}Temperature\\ Control\\ System\end{tabular}}} & $T_O$ \textless 0 or 60 \textless $T_O$                                                                                                            & \multirow{-3}{*}{\%99.9}       \\ \hline
		\multicolumn{1}{|c|}{\cellcolor[HTML]{C0C0C0}}                                                                                         & $-\epsilon + |\rho| <$  0.1 \& $\epsilon < 0.2$ \& $|\rho| < \pi/8 $                                                                                                           &                                \\ \cline{2-2}

		\multicolumn{1}{|c|}{\cellcolor[HTML]{C0C0C0}}                                                                                         & 0.2$< -\epsilon + |\rho| <$  0.1 \& $0.2<\epsilon < 0.3$                                                                                         &                                \\
		\multicolumn{1}{|c|}{\cellcolor[HTML]{C0C0C0}}                                                                                         & \& $\pi/8 < |\rho| < \pi/6$                                                                                                           &                                \\ \cline{2-2}
		\multicolumn{1}{|c|}{\multirow{-5}{*}{\cellcolor[HTML]{C0C0C0}\begin{tabular}[c]{@{}c@{}}3DOF\\  Helicopter\end{tabular}}}             & $ -\epsilon + |\rho| <$  0.2 \& $0.3<\epsilon$ \& $\pi/6 < |\rho| $                                                                                                           & \multirow{-5}{*}{\%64.3}       \\ \hline
	\end{tabular}
\caption{Weighted average availability of the embedded system.}
	\label{table:availability}
\end{table}



==> for arXiv/Sections/framework_overview.tex <==
\section{Restart-Based Security: An Overview}
\label{subsec:res-overview}


Immediately after a reboot, if all the external interfaces have remained disabled and if the software is loaded from a read-only storage, system can be considered as uncorrupted.  




\hl{In light of this observation, restarting the system is independent of previous actions of attackers and it is guaranteed to put the system in hands of the desired uncorrupted software.} \todo[inline]{@Fardin: not very clear. please rephrase -MH}


\begin{figure}[ht]
	\begin{center}
		\includegraphics[width=0.49\textwidth]{flow}
		\caption{Sequence of the events within one restart cycle.}
		\label{fig:eventorder}
	\end{center}
\end{figure}

%With this in mind, 

The high-level overview of the proposed approach is illustrated in Fig.~\ref{fig:eventorder}).
One of the core components of our approach is to use \textit{safety controller}~(SC) that stables the system during restart\footnote{The idea of safety controller is elaborated in Section \ref{sec:background}.}.
 The key idea is that, after a reboot (while the software is still uncompromised) the time of next restart must be decided such that the following conditions remain satisfied:

\begin{itemize}
 %\ci 
 \item From current time instant until the completion of the next reboot, state will remain inside the admissible region even if the adversary is in full control; and  
 %\cii
 \item  The state of the plant after completion of the next reboot is such that the SC can stabilize the system. 
\end{itemize}


The sequence of events illustrated in Fig.~\ref{fig:eventorder}) are repeated after every restart. However, at any point of time, if state is so close to the boundary of the admissible and inadmissible states such that there is no tolerance for adversarial control~(\ie if adversary takes over can crash the in very very short time), the SC remains in charge for longer and pushes the plant further into the set of admissible states $\mathcal{S}$ (refer to Section~\ref{sec:background}) until the safety margin is large enough.  


==> for arXiv/Sections/implementation.tex <==
\section{Implementation and Attacks}

\label{sec:implementation}

Now, we present an overview of our prototype implementation of a restart-based protection approach for the control embedded system of an \emph{actual} 3DOF helicopter platforms. More detailed description on the implementation is given in our technical report~\cite{githubrepoemsoft}. In addition, through \emph{hardware-in-the-loop} approach, we use the same embedded system for controlling the warehouse temperature system. We test some attacks on both system and verify that the safety requirements are respected. 

\begin{figure}[ht]
	\begin{center}
		\includegraphics[width=0.45\textwidth]{lab}
		\caption{3DOF helicopter used as the test-bed.}
		\label{fig:3dof}
	\end{center}
\end{figure}


\subsubsection*{RoT Module:}
We implemented the RoT module using a minimal MSP430G2452 micro-controller on a MSP-EXP430G2 LaunchPad board~\cite{launchpadboard}. 
To enable restarting, pin P2.0 of the micro-controller is connected to the restart input of the main controller. Internal \emph{Timer A} of the micro-controller is used for implementing the restart timer. It is a 16-bit timer configured to run at a clock rate of 1MHz (\ie $1\mu s$ per timer count) using the internal digitally controlled oscillator. A counter inside the interrupt handler of \emph{Timer A} is used to extend the timer with an adjustable factor, in order to enable the restart timer to count up to the required range based on the application's needs.

The $I^2C$ interface is adopted for the main controller to set the restart time on RoT module. After each restart, RoT acts as an $I^2C$ slave waiting for the value of the restart time. As soon as the main controller sends the restart time, RoT disables the $I^2C$ interface and activates the internal timer. Upon expiration of the timer, an active signal is set on the restart pin to trigger the restart event and the $I^2C$ interface is activated again for accepting the next restart time.

\subsubsection*{Main Controller:}
We used a Zedboard~\cite{zboarddatasheet} to implement the main controller of the 3DOF helicopter and warehouse temperature control system. Zedboard is a development board for Xilinx's Zynq-7000 series all programmable SoC. 
It contains a XC7Z020 SoC, 512MB DDR3 memory and
an on-board 256MB QSPI Flash.
The XC7Z020 SoC consists of a processing system (PS) with dual ARM Cortex-A9 cores and a 7-series programmable logic (PL).
The processing system runs at 667MHz.
In this evaluation, only one of the ARM cores is used while the idle one is not activated.
The programmable logic is programmed to provide the $I^2C$ and \emph{UART} interfaces that are used for connecting to the RoT module and the 3DOF helicopter.

%===== FreeRTOS and tasks =====
The main controller runs \emph{FreeRTOS}~\cite{FreeRTOS}, a preemptive real-time operating system. Immediately after the reboot when the \emph{FreeRTOS} starts, \texttt{SafetyController} and \texttt{FindRestartTime} tasks are created and executed. \texttt{SafetyController} is a periodic task with a period of $20ms$~($50Hz$). And, \texttt{FindRestartTime} is a single task that executes in a loop, and it only breaks out when a positive restart time is found. At this point, the restart time is sent to the RoT module via $I^2C$ interface, \texttt{SafetyController} and \texttt{FindRestartTime} tasks are terminated and the main control application tasks are created. To calculate reachability in run-time in function \texttt{FindRestartTime}, we used the implementation of real-time reachability approach in~\cite{rt-reach}.

%===== reset and boot process =====
Reset pin of Zedboard is connected to RoT module's reset output pin.
The entire system (both PS and PL) on Zedboard is restarted when the reset pin is pulled to low state.
The boot process starts when the reset pin is released (returning to high state).
A boot-loader is first loaded from the on-board QSPI Flash.
The image for PL is then loaded by the boot-loader to program the PL which is necessary for PS to operate correctly.
%This step takes 100ms in minimum.
Once PL is ready, the image for PS is loaded and \emph{FreeRTOS} will take over the control of the system.

%===== Randomization =====
To further enhance the security of \emph{FreeRTOS}, we adopt \emph{randomization techniques} to randomize the following attributes: 
\ci the order of the task creation and \cii task scheduling.
After every restart, we randomize the order of creating the application tasks.
By doing so, the memory allocation is somewhat shuffled as the memory blocks are assigned to the tasks dynamically when they are created in \emph{FreeRTOS}.
Additionally, we port \emph{TaskShuffler}, a schedule randomization protocol~\cite{taskshuffler}, on \emph{FreeRTOS}.
This technique randomly selects a task from the scheduler's ready queue to execute, subject to each task's pre-computed priority inversion budget, at every scheduling point. Randomizing system parameters increases the difficulty of launching the same attack after each restart.

\textbf{3DOF Helicopter Controller:} The main controller unit interfaces with the 3DOF helicopter through a PCIe-based \textit{Q8 High-Performance H.I.L. Control and data acquisition unit}~\cite{q8daq} and an intermediate Linux-based PC. The PC communicates with the ZedBoard through the serial port. At every control cycle, a task on the controller communicates with the PC to receive the sensor readings~(elevation, pitch, and travel angles) and send the motors' voltages. The PC uses a custom Linux driver to send the voltages to the 3DOF helicopter motors and reads the sensor values. The code for the controller including the controllers and optimizations to reduce the boot sequence of ZedBoard is available online~\cite{githubrepoemsoft}.

\textbf{Warehouse Temperature Controller:} For system, due to lack of access to the real physical plant we used a hardware-in-the-loop approach. Here, the PC runs a simulation of the temperature based on the heat transfer model of Equation~\ref{eq:heatermodel1} and~\ref{eq:heatermodel2}. Similar to the 3DOF helicopter, the controller is implemented on the ZedBoard with the exact same configuration~(RoT, serial port connection, I$^2$C interface, $50Hz$ frequency) as described earlier. Control commands are sent to the PC, applied to the system and the state is reported back to the controller.


% 
%
%\begin{table}[!htb]
%	%\renewcommand{\arraystretch}{1.2}
%	\caption{Implementation Platform and Experimental Parameters}
%	\label{tab:ex_param}
%	\centering
%	%\begin{tabular}{c||p{5.9cm}}
%	\begin{small}
%		\begin{tabular}{p{3.5cm}||p{4.15cm}}
%			\hline %\\
%			\bfseries Artifact/Parameter & \bfseries Values\\
%			\hline\hline
%            RoT Module & MSP-EXP430G2 LaunchPad \\ & MSP430G2452 \\
%            Main Controller Platform & Zedboard \\ & XC7Z020, 512MB RAM \\
%            Main Controller OS & FreeRTOS \\
%            Reboot Time, $T_R$ & $390~\rm{ms}$ \\
%			\hline
%		\end{tabular}
%	\end{small}
%\end{table}

\subsection{Attacks on the Embedded System}

To evaluate the effectiveness of the proposed approach, we tested three types of  synthetic attacks on the implemented controller of the 3DOF helicopter with actual plant and one attack on the hardware-in-the-loop implementation of the warehouse temperature control system.In these experiments, our focus is on the actions of the attacker after the breach into the system has taken place. Hence, the breaching approach and exploitation of the vulnerabilities is not a concern of these experiments. 


In the first attack experiment, we evaluate the protection provided by our approach in presence of an attacker who, once activated, is capable of killing the main controller task. The attack is activated at a random time after the end of SEI. We observed that under this attack, the 3DOF helicopter did not hit the surface~(\ie it always remained within the set of admissible states). 


In the second attack experiment, attacker replaces the sensor readings of the system with corrupted values with the aim of destabilizing the plant and reducing its progress. The activation time of this attack, similar to the previous one, is dictated by a random variable. Similar to the first attack experiment, system remained safe throughout the attacks. And the progress of the system was negatively impacted for as the activation time of the attack became smaller. 


In the third attack experiment, we investigate the impact of a \emph{worst-case} attacker who becomes active immediately after the SEI and replaces the original controller with a malicious process that turns off the fans of the helicopter leading it to hit the surface. We observed that the system was able to tolerate this attack and did not hit the surface. The trace of the system during a time interval of activity is plotted in Figure~\ref{fig:traceofattack}. 

From figure, it can be seen the controller spends most of the time in SEI~(red region) or in reboot~(white region). This is due to the fact that this extreme-case attack is activated immediately after each SEI and destabilizes the helicopter. By the time that the reboot is complete~(end of the white region), system is close to unsafe states. Hence, SEI becomes longer as SC is stabilizing the system. under this very extreme attack model, the system does not make any progress towards its designated path under this attack model. 


\begin{figure}
\includegraphics[width=0.48\textwidth]{3dof-worst-case-demo}
\caption{Trace of 3DOF Helicopter during two restart cycles when the system is under worst-case attack that is active immediately after SEI. Green: SEI, red: system reboot, white: Normal Operation~(In this case attacker)}
\label{fig:traceofattack}
\end{figure}

In the last experiment, an attack is performed on the embedded controller of the warehouse temperature. In this experiment, the outside temperature is set to $45^\circ C$ and initial temperature of the room is set to $25^\circ C$. The attacker takes full control of the system and immediately after the SEI, activates both heaters to increase the temperature. We observed that system restarts before the room temperature goes above $30^\circ C$ and after the restart, SC drives the temperature towards the safe range.
















==> for arXiv/Sections/introduction.tex <==
\section{Introduction}

Conventionally, embedded cyber-physical systems (CPS) used custom platforms, software/protocols and were normally not linked to external networks. As a result, security was typically not a priority in their design.
However, due to the drive towards remote monitoring and control facilitated by the growth of the Internet along with the increasing use of common-off-the-shelf (COTS) components, these traditional assumptions are increasingly being challenged as evidenced by recent attacks \cite{dronhack, ris_rts_1, 5751382}. Any successful, serious attack against such systems could lead to problems more catastrophic than just loss of data or availability because of the critical nature of such systems \cite{checkoway2011comprehensive,gollakota2011they}.


One of the challenges of designing secure embedded systems is to develop techniques/frameworks that consider the safety requirements of any physical system that they may control and operate within resource-constrained environments of embedded platforms. In the design of such a secure framework, it is important to distinguish between \textit{physical safety} and \textit{cyber-security}. For many embedded systems, violation of cyber-security~(\eg stealing system secrets, logging user activity pattern, taking control of the system, \etc) by itself may not be considered as harmful as violation of physical safety~(\eg destabilizing a helicopter by moving towards other objects or ground). %filling a gas tank beyond its pressure capacity or increasing temperature of a food warehouse above the safe range). 
In fact, in the context of embedded CPS, one of the goals of an adversary could be violate physical safety eventually and cause physical damage. Unfortunately, many of the existing security techniques are designed for traditional computing systems and do not take into the account the physical aspect of embedded systems. Hence, they are not always effective in ensuring physical safety in the presence of attacks.


On one hand, many existing security mechanisms aim to protect against malicious activities and/or detecting them as quickly as possible. It is, however, not easily possible to detect or protect from \textit{all} the attacks without any false negatives. On the other hand, safety guarantees verified by design methods for safety-critical CPS are only valid for the original uncorrupted system software. In other words, \textit{if security of the system can not be guaranteed, safety requirements may also be broken}. 
%Besides, introducing additional complexity to improve security results in the increased difficulty for the verification of the system components (\eg application software, firmware, OS, \etc) and may increase downtime. 
Hence there is need for security mechanisms that are specifically designed for safety-critical systems with verifiability in mind.

In this paper, we propose a design method for safety-critical embedded CPS that \textit{decouples physical safety} from \textit{cyber security}, \ie it guarantees the safety of the physical system even when the security of the embedded system cannot be guaranteed. 
%Due to \textit{inertia}, pushing a physical plant from a given (potentially safe) state to an unsafe state -- even with complete adversarial control -- is not instantaneous and often takes finite (even considerable) time. 
 The main idea of the paper is based on two key observations. \textit{First,} restarting a computing unit and reloading the software from a protected storage is an effective way to remove any malicious component from the system (albeit for a short, finite amount of time) and restore the software to an uncorrupted, functional condition~\cite{mhasan_resecure16}. \textit{Second,} physical systems, unlike computing systems, have \textit{inertia}. As a result, changing the state of a physical plant from a safe state to an unsafe one even with complete adversarial control\footnote{For instance if the adversary gains root/administrative access in the system.} is not instantaneous and takes considerable time (\eg increasing temperature, increasing pressure, \etc) We leverage
	this property to calculate a \textit{safe operational window} and combine it with the effectiveness of {\em system-wide
		restarts} to decrease the efficacy of malicious actors.



In our approach, the power of system-restarts is used to \textit{recover the embedded system from a potentially corrupted condition to a trusted and functional state}. At this point, all external interfaces~(\eg network and debugging interface) of the embedded system (except for the sensors and actuators) are disabled. While system is in this isolated mode, a safe operational window is calculated during which, even with full control of the adversary, the physical plant cannot reach an unsafe state. In this isolated mode the next restart time of the embedded system is also set dynamically. Then, the main controller and all interfaces are activated and system starts the normal operation until the restart time time is reached. This process repeats after each restart. However, if at some point, the plant is too close to the safety boundary such that calculated safety window is too short~(\ie system cannot tolerate any adversarial behavior), the secure/isolated operational mode is extended. During the extended period,  a \textit{safety controller (SC)} drives the plant towards the safe states and farther away from the unsafe boundary. Once the system has a reasonable margin, next restart time is set and normal controller is activated. In our design, \textit{an external isolated simple hardware module} acts as the \emph{Root of Trust~(RoT)}\footnote{The proposed RoT module can be constructed using simple commercial off-the-shelf~(COTS) components.} and triggers the restarts (Section \ref{sec:RoTDesign}). This guarantees that even very strong adversaries cannot interfere with the system restart events.


%However, security still remains an important factor as it directly impacts availability and progress of the CPS towards the mission. 


%\todo[inline]{IMPORTANT: the intro (and also beginning of section 4) needs a few sentences of WHY restart based mechanisms work! The idea that it will kick the attacker out, has to start again etc. So far this is missing.}



Notice that only restarting the embedded platform may make it easier for the attacker to penetrate the system again. However the dynamic calculation of restart times and other quantities (\eg reachability calculations, see Section \ref{sec:securetime}) makes it harder for the attacker to succeed. Along with restart, using the approaches described in Section \ref{sec:discussion}, it is possible to further increase the difficulty for the attacker to intrude and cause damage to the system.

Note that with optimizing the boot sequence and given the embedded nature of such systems, \textit{the time required to restart and reload the software can be very short}. The impact of the proposed approach on availability of the system varies according to the boot time of the particular embedded system~(type of the OS, processor, storage, size of the software, \etc) and the physical plant's dynamics~(that determines the rate of restarts).  Such an impact is negligible for systems with slower dynamics such as temperature control system and it can increase for unstable systems such as avionics (see Section~\ref{sec:evaluation}). Figure~\ref{fig:applicableFields} illustrates the impact of the proposed approach on some categories of applications, in an abstract sense.

\begin{figure}[ht]
	\begin{center}
		\includegraphics[width=0.35\textwidth]{applicable_fields.pdf}
		\caption{Impact of the proposed restart-based protection increases with the Speed of dynamics of the physical sub-system.}
		\label{fig:applicableFields}
	\end{center}
\end{figure}

 


%The main contributions of this paper can be summarized as follows:
In this paper we make following contributions:
\begin{itemize}
	\item We propose an approach to calculate the safe operation window for CPS and hence, improve its overall security. By utilizing system-wide restarts the proposed framework can recover a potentially compromised system. (Section~\ref{sec:probability}).
    \item We guarantee the safety of the physical system despite security threats (Section~\ref{sec:details}).
	\item  We demonstrate the effectiveness of our proposed method using a proof-of-concept implementation as applied to realistic systems (Section~\ref{sec:evaluation}).
\end{itemize}


\begin{comment}

Note: Sibin don't like this way -- MH.
This paper is organized as follows. Section~\ref{sec:model} reviews the system model and adversarial capabilities. Section~\ref{sec:method} provides an overview of the approach and a brief background on safety controller. In Section~\ref{sec:details}, restart-based protection is discussed in detail. In Section~\ref{sec:probability}, we elaborate on the impact of periodic restarts on improving security of the system. We evaluate the approach using two physical systems in Section~\ref{sec:evaluation}. We discuss some limitations and considerations of the approach in Section~\ref{sec:discussion} and provide a brief overview of the related work in Section~\ref{sec:related}. Section~\ref{sec:conclusion} concludes the paper.
\end{comment}

%We also introduce the concept of \emph{Secure Execution Intervals}~(SEI). Every SEI is a fixed short interval after each restart during which system operates in an isolated manner and does not interact with any external entity except sensor readings. During SEI we propose external interfaces (such as network and debugging interfaces). Due to the fact that the software running on the system is guaranteed to remain uncompromised during SEI time slots, the execution can be trusted and assumed secure. 



% To be specific, SEI can be considered as a Time division multiple access~(TDMA) for dividing system resources between secure and insecure execution intervals. 
 
% There exists security techniques that introduce additional isolated hardware modules to ensure trusted execution of monitoring tasks for intrusion detection~\cite{securecore, slack_cornell}% and health monitoring~\cite{cite something else}. 
%Our approach, in contrast, achieves a similar goal \textit{without} utilizing any extra hardware. 




==> for arXiv/Sections/limitations.tex <==
\section{Discussion}
\label{sec:discussion}

%\textit{Suitable Application Targets}: 
\textbf{Suitable Application Targets:} Restart-based protection aims to provide a very strong protection guarantees for the CPS. However, it is not necessarily applicable to every system. The main limiting factor is the speed of the dynamics of the physical plant and the restart time of the embedded platform. Physical systems that are unstable, have very narrow safety margin, or have very fast moving dynamics have a very low tolerance for misbehavior. Adversaries can damage such systems very quickly. As a result, applying restart-based protection to such systems would require them to restart very fast. Very fast restart rates may reduce the controller's available time and essentially prevent the system from making any progress. It may also create implementation challenges; a system may require some time to establish connection over Internet or to authenticate that may not be possible if the system has to restart very frequently. Therefore, before adapting the proposed mechanism for a system, a set of tests similar to the evaluations in Section~\ref{sec:restarttimeeval} need to be performed to check if the restart times are within a suitable range. On the other hand, systems with slower dynamics and winder safety margins~(\eg Internet of Things~(IoT) applications, infrastructure, municipal systems, transportation, and \etc) are the most suitable category to benefit from this technique. 


%\textit{Threat Model}: 


\textbf{Threat Model:} The restart-based approach proposed in this paper provides guaranteed protection for the physical sub-system in presence of the attacks. However, attackers may cause other forms of damage to the system that are not physical; \eg attacks targeting performance of the system, logging and stealing information, and man-in-the middle attacks. Even though such attacks are not the main focus of this paper, a similar approach to the analysis of Section~\ref{sec:probability} can be performed to evaluate the effectiveness of restart-based protection on mitigating the impact of such attacks.



%\textit{Increasing the Entropy}:



\textbf{Increasing the Entropy:} Despite the effectiveness of restarting and software reloading in removing the malicious components from the system, restarting does not fix the vulnerabilities of the system that provided the opportunity for the intruder to breach into the system. An attacker maybe able to re-launch the same attack after the restart and gain control of the system. It turns out, randomizing parameters and operation of the system introduces a noise in the execution pattern of the system within each cycle, thereby, increasing the time and effort needed by the attacker to trigger the attack. In other words, randomization reduces the impact of previous knowledge in launching new attacks. There is a considerable body of work on various randomization techniques for security protection; \eg schedule Randomization~\cite{taskshuffler}, address space randomization~(ASLR)~\cite{Shacham:2004:EAR:1030083.1030124}, and Kernel Address Space Randomization~(KASLR)~\cite{Jang:2016:BKA:2976749.2978321}.



%For a malicious activity to be successful, usually, an attacker needs a set of information about the system \eg execution trace of system to perform side-channel attack and break a cryptographic key~\cite{cite a paper} and memory address of particular functions for Return-to-libc attack~\cite{cite a paper}. 






==> for arXiv/Sections/methodology.tex <==
\section{Restart-Based Protection}
\label{sec:details}



%Immediately after a reboot, if all the external interfaces have remained disabled and if the software is loaded from a read-only storage, system can be considered as uncorrupted.  

The goal of our proposed restart-based security approach is to \textit{prevent adversaries from damaging the physical plant}. The high-level overview of the proposed approach is illustrated in Fig.~\ref{fig:eventorder}.
The key idea is that, after a reboot (while the software is still uncompromised) the time instant to initiate the next restart must be decided such that the following conditions remain satisfied:

\begin{itemize}
	%\ci 
	\item From the current time instant until the completion of the next reboot state will remain inside the admissible region even if the adversary is in full control and  
	%\cii
	\item  The state of the plant after completion of the next reboot will be such that the SC can stabilize the system. 
\end{itemize}


\begin{figure}[!tb]
	\begin{center}
		\includegraphics[width=0.40\textwidth]{flow}
		\caption{Sequence of the events.}
		\label{fig:eventorder}
	\end{center}
\end{figure}



After every restart (Marker VIII in Fig.~\ref{fig:eventorder}), the goal is to set the time of the next restart (Marker VII) such that it satisfies the above conditions (Marker VI). However, if the physical plant's state is too close to the boundary between the admissible and inadmissible states, there may not exist a time value that satisfies these conditions -- since, in such states, the system has no tolerance for unexpected behavior and if the adversary takes over, it can damage the plant in a very short time.
In such cases, the SC remains in charge of the control (illustrated by Marker V) for longer time and pushes the plant further into the set of admissible states $\mathcal{S}$ (refer to Section~\ref{sec:background}) until the safety margin is large enough and the restart time can be calculated~(system moves back and forth between states IV and VI until a restart time is available). 

% done this one



%$l_r$ is the upper bound of the restart time of the platform. Throughout this paper, we assume that $l_r$ is fixed for the given platform and cannot be changed. $T_r$ is the period of the restart of the system. This is the interval after which we want the system to restart, and can be decided by the system during the trusted interval. $T_t$ is the length of trusted interval. 



%\ci providing a \textbf{minimum guaranteed} execution frequency of the safety checks and health monitoring tasks \cii enable the nodes to send out reliable uncorrupted data to the central coordinator or other nodes with a \textbf{guaranteed minimum period}, \ciii provide a minimum \textbf{guaranteed progress} towards the control task. 

\begin{comment}

The key observation that enables our design is the fact that immediately after a reboot, if all the external interfaces have remained disabled, and if the software is loaded from a read-only storage, system can be assumed to be  uncorrupted.  In light of this observation, restarting the system, independent of previous actions of attackers, is guaranteed to put the system in hands of the desired uncorrupted software. 

\begin{figure}[ht]
	\begin{center}
		\includegraphics[width=0.49\textwidth]{events}
		\caption{Sequence of the events within one restart cycle.}
		\label{fig:eventorder}
	\end{center}
\end{figure}

With this in mind, our high-level approach~(Figure~\ref{fig:eventorder}) is that after a reboot, while the software is still uncorrupted, the time of the next restart must be decided such that the following conditions remain satisfied; \ci from now until the completion of the next reboot, state will remain inside the admissible region even if the adversary is in full control. \cii state of the plant after completion of the next reboot is such that the SC can stabilize the system. This process repeats after every restart. However, at any point, if state is so close to the boundary of the admissible and inadmissible states such that there is no tolerance for adversarial control~(\ie if adversary takes over can crash the in very very short time), the SC remains in charge for longer and pushes the plant  further into the $\mathcal{S}$ until the safety margin is large enough.  


\end{comment}


Three challenges need to be addressed for this approach to be practical. First, we need a \textit{mechanism to compute the next restart time after each reboot}. Second, we need to \textit{ensure the integrity of the process that performs this computation}. Third, once the next restart time is computed, \textit{a mechanism is needed to enforce its execution at designated time despite full adversarial control of the embedded system}. 

To address the first challenge, an approach for computing the safe restart time (Marker V in Fig.~\ref{fig:eventorder}) is presented in Section~\ref{sec:securetime}. To guarantee integrity of restart time computation~(second challenge), we introduce the idea of \textit{secure execution intervals~(SEI)} as illustrated by Marker III in Fig~\ref{fig:eventorder}. After every restart, for a short interval of time, all the external interfaces of the system remain disabled (Marker II). This allows the reliable execution of SC and for trusted computation of the restart time without adversarial interference. SEI is discussed in more detail in Section~\ref{sec:SEI}. Furthermore, to ensure that the intruder cannot prevent the system from restarting~(third challenge), the design includes a simple, isolated hardware module (illustrated by Marker I) called~\emph{Root of Trust~(RoT)} discussed in Section~\ref{sec:RoTDesign}. 


%Mechanisms described so far, guarantee the safety of physical system despite the possible threats. However, adversaries still may be able to launch attacks after restarts slow down progress of the system. As a result, we include a progress monitoring task during the SEI which evaluates the progress of the system using the physical measurements and available signals such as battery/fuel level, GPS and etc. If any abnormality is detected, the restart time is further reduced. Such a feedback-based mechanism, reduces the restart time to the point where the attacker cannot launch its attack and therefore the progress of the system remains untouched. To support the monitoring task, an additional secure memory unit is included in the RoT which provides read/write access only during the SEI. This memory unit is used to securely store operation traces and other information required to perform the progress evaluation. 


%During the intervals, system can execute some safety checks to ensure that the system is not in an unsafe state. Furthermore, through health-checking mechanism using the sensor values and previous measurements system can evaluate the progress factors and decide on the next course of action. In the rest of this section, we discuss more details regarding these components. 


%The first idea of restart-based security is that if the system is restarted \textit{frequently enough}, it is less likely that the attacker will have time to trigger the attack and cause meaningful damage to the system. After every restart, there will be a predictable down time (during the system reboot), some operational time (before system is compromised again) and some compromised time (until the compromise is detected or periodic timer expires). The expected amount of time that the system is under the attack can be reduced by adjusting the external restarting period. 


%The length of each one of the above intervals depends on the type and configuration of the platform, adversary models, effectiveness of the monitoring unit and complexity of the exploits. As a general rule, the effectiveness of the restarting mechanism increases \textit{i}) as the time to re-launch the attacks increases or \textit{ii}) the time to detect attacks and trigger a restart decreases. In the Appendix, we provide a probabilistic method\footnote{A similar probabilistic analysis is performed in literature \cite{huang1995software} to find the optimal restart time for software rejuvenation purposes.} to evaluate the expected unavailability due to restarts and attacks and the expected damage from the attacks/exploits given a certain restart configuration. We also show how to find an optimal configuration to balance lack of availability and damage.

% In these figures, $T_R$ is the time for a full complex unit restart, $T_{Com}$ is the time the attacker needs to re-launch the attack~(During this time system is not compromised yet), $T_{Detect}$ is the time it takes for the monitoring unit to detect the attack and initiate a restart; $T_{Timer}$ is the fixed time for the periodic timer to restart the system. 

% Figure~\ref{fig:detect-restart} illustrates the case when the monitoring unit detects the attack before the periodic timer expired ($T_{Detect} +  T_{Com}< T_{Timer}$), whereas 

% in Fig.~\ref{fig:timer-restart}, periodic timer expires before the monitoring unit detects the attack ($T_{Detect} + T_{Com} > T_{Timer}$). 


% \begin{figure}[h!]
%   \centering 
%   \subfigure[%A restart, followed by a compromise and detection restart
%   ]{\label{fig:detect-restart}\includegraphics[width=0.31\textwidth]{attack1}}
%   \subfigure[%A restart, followed by a compromise and a HW timer restart
%   ]{\label{fig:timer-restart}\includegraphics[width=0.36\textwidth]{attack2}}
%   \caption{%A restart, followed by a compromise and a HW timer restart
%   Flow of operation during intrusion: (a) a restart, followed by a compromise and detection restart; (b) a restart, followed by a compromise and a periodic timer restart.}
% \end{figure}



It is useful to define some parameters before the detailed discussion on the components. In the rest of this section, $T_s$ is the length of the SEI and is fixed throughout operation, and $t$ is the current time. In addition, $T_r$ is the time it takes for the embedded system to restart and reboot.

\subsection{Secure Execution Interval~(SEI)}
\label{sec:SEI}

The need for SEIs arises from the fact that a mechanism is required to prevent any malicious interference towards the tasks that are necessary for providing the safety guarantees. After a restart, while all the external interfaces of the system remain disabled, the system software is loaded into memory from a read-only storage unit. Disabling interfaces isolates the system and protects it from intruders. So long as the system is isolated, we assume that the software is uncorrupted. SEI refers to this isolated interval of time after each restart. %until the restart time is calculated and set on RoT.

During the SEI, two tasks execute in parallel: SC (which runs periodically to keep the physical system stable) and \texttt{FindRestartTime} (Section~\ref{sec:securetime}). If \texttt{FindRestartTime} cannot find a safe restart time~(this may occur when the physical plant is very close to being in the  inadmissible region), SEI is extended for another $T_s$ time units\footnote{As we illustrate in Section~\ref{sec:evaluation}, this extension does not negatively affect the safety.}. Extending SEI gives SC more time to push the state further away from the unsafe boundary and into the admissible region. If \texttt{FindRestartTime} task is able to find a restart time, \ca the \texttt{SetRestartTime} interface of the RoT~(details in next section) is used to set the time for the next restart event, \cb SEI terminates, \cc all the interfaces are activated, \cd the main controller of the system is activated and \ce the  system enters normal operation mode -- until the next restart takes place. Note that following this procedure, the \texttt{SetRestartTime} interface of RoT will be called exactly \emph{once} before the SEI terminates.


\subsection{Hardware Root of Trust~(RoT)}
\label{sec:RoTDesign}

Our design requires a mechanism to ensure that under any circumstances, the adversary cannot prevent the system from restarting. Hence, we include an isolated HW module in charge of triggering restarts and refer to it as hardware root of trust~(RoT).

RoT provides a hardware interface, $\texttt{SetRestartTime}$, that during the SEI allows the processor to set the time of the next restart event.  To achieve this, after each restart, RoT allows  the processor to call the \texttt{SetRestartTime} interface only \emph{once}. Additional calls to this interface will be ignored. RoT immediately sets a timer for the time value received from \texttt{SetRestartTime} interface and issues a restart signal to the hardware restart pin of the platform upon its expiration.

	
%	\item  RoT contains a memory unit and provides two protected interfaces \texttt{write(addr, val, size)} and \texttt{read(addr, val, size)}. These interfaces are protected, meaning that \texttt{read} and \texttt{write} requests are executed only if system is in the SEI	otherwise ignored \ie $t-t_0 \leq \delta_t$ where $t$ is the time of the request.


In order to achieve the security goals of the platform, ROT needs to be secure and incorruptible. Hence, we require hardware isolation~(\eg a standalone timer) and independence from the processor with no connectivity except for the HW interface \texttt{setRestartTime}. In our prototype implementation, RoT is implemented using a simple micro-controller (Section~\ref{sec:evaluation}).

%
%\begin{figure}[ht]
%	\begin{center}
%		\includegraphics[width=0.49\textwidth]{trusted-hw}
%		\caption{Restart Unit TODO: update the figure and remove the core}
%	\end{center}
%	\label{fig::rot}
%\end{figure}
%
%The logical design presented in Figure~\ref{fig::rot} can be used as an instance implementation. The design consists of two timers (T1 and T2) and a memory unit. In this design, T1 is in charge of keeping track of the restart period $T_r$ and issuing the restart command to the restart pin of the processor. T2 in this design, is in charge of measuring the time for the trusted interval. After $T_r$ elapsed, T1 expires and it simultaneously triggers a restart to the processing unit and starts the count down on T2. T2 is initialized with the a fixed value of $T_t$. During the count down, the T2 outputs an active signal on the output pin. This signal is connected to the \texttt{WRITE\_ENABLE} pin of the memory and and \texttt{SET\_ENABLE} pin of the timer. \texttt{MEM\_ENABLE} allows the processor to read from and write into memory. Furthermore, T2 activates the \texttt{SET\_ENABLE} pin which enables the processor to set a new $T_r$ on as T1's initial value. 




\subsection{Finding a Safe Restart Time}
\label{sec:securetime}
%One of the main challenges to address in this paper is the problem of guaranteeing safety under the attacks. In particular, given the adversary model we have assumed, attacker can crash or modify any of the components in the system after the restart period is over. Such a strong adversary can maliciously corrupt the safety controller and generate commands that eventually take the physical system to an state beyond recovery. This is not acceptable for a safe system. In other words, the goal of our system is to prevent the attacker to every being able to take the system into an unrecoverable state. In this section, we demonstrate how such a goal is achieved. 



%During the SEI, the next restart time of the system needs to be set using the \texttt{set\_restart} interface of RoT. The idea is to set the next restart time such that, the system is guaranteed to stay within admissible states until the restart. To achieve this, we utilize the inertia of physical systems. 


%Unlike computational systems, physical components have inertia and their state is a continuous variable that gradually changes over the time. As a result, if state is inside the admissible region, an attacker with full control of the computational unit, would still need some time to take the system into an inadmissible/unsafe state. In this section, we demonstrate how to calculate the minimum time required for a physical system to reach an unrecoverable state from a given state. 


In this section, we now discuss the implementation of the \texttt{FindRestartTime} task. This task is activated immediately after system reboot, along with the SC task  and calculates the time for the next restart event.

Before we proceed, it is useful to define some notations. We use the notation of $\mathsf{Reach}_{=T}(x,C)$ to denote the set of states that are reachable by the physical plant from an initial set of states $x$ after exactly $T$ units of time have elapsed under the control of controller $C$~\cite{rt-reach}. $\mathsf{Reach}_{\leq T}(x,C)$ can be defined as $\bigcup_{t=0}^{T} \mathsf{Reach}_{=t}(x,C)$ \ie set of all the states reachable within up to $T$ time units. In addition, we use $SC$ to refer to the \emph{safety controller} and $UC$ to refer to an \emph{untrusted controller}, \ie one that is compromised by the adversary.

Conditions presented in our newly developed Theorem~\ref{thm:safety} evaluates whether the system remains safe and recoverable if restarted after $\delta_r$ time units.

\begin{theorem}
Assuming that $x(t)$ is the state of the system at time $t$ and the adversary controls the system~(UC) from $t$ until the restart of the system. Under the following conditions, the embedded system can be restarted at time $t + \delta_r$ thus guaranteeing that attacker cannot violate the safety requirements of the physical plant:
\begin{enumerate}
	\item $\mathsf{Reach}_{\leq \delta_r + T_r}(x, UC) \subseteq
	\mathcal{S}$\label{cond:hardconst_reach_pre_tc};
	\item $\mathsf{Reach}_{\leq T_\alpha}(\mathsf{Reach}_{= \delta_r + T_r}(x, UC), SC)
	\subseteq \mathcal{S}$\label{cond:hardconst_reach_pre_ts};
	\item$\mathsf{Reach}_{= T_\alpha }(\mathsf{Reach}_{= \delta_r+T_r}(x, UC), SC)
	\subseteq \mathcal{R}$\label{cond:hardconst_reach_ts}.
\end{enumerate}
\label{thm:safety}
\end{theorem}

\begin{proof}
Intuitively, this condition says that plant remains safe if, \ca the adversary~(UC) cannot reach an inadmissible state before the next restart completes ($\delta_r + T_r$), \cb if the safety controller takes over after next restart, it will avoid unsafe states until $\delta_r + T_r + T_\alpha$ time units passes and \cc after $\delta_r + T_r + T_\alpha$ time, a state in $\mathcal{R}$ will be safely reached.
	
	
To prove formally, assume by contradiction that the system is not safe under these conditions. Hence, an inadmissible state is reached at some time. This time will be either less than $\delta_r + T_r$, more than $\delta_r + T_r$ and less than $\delta_r + T_r + T_\alpha$ or more than $\delta_r + T_r + T_\alpha$. The first two of these cases are ruled out directly by conditions (1) and (2), so only the third case needs to be examined.

From properties of SC, $\mathsf{Reach}_{\leq \infty}(\mathcal{R}, SC) \cap \mathcal{S}' = \emptyset$. Since if $\mathcal{R}' \subseteq \mathcal{R}$, $\mathsf{Reach}_{\leq \infty}(\mathcal{R}', SC) \subseteq \mathsf{Reach}_{\leq \infty}(\mathcal{R}, SC)$, the smaller set of states $\mathcal{R}' = \mathsf{Reach}_{= T_\alpha }(\mathsf{Reach}_{= \delta_r+T_r}(x, UC), SC) \subseteq \mathcal{R}$ will also satisfy the condition $\mathsf{Reach}_{\leq \infty}(\mathcal{R}', SC) \cap \mathcal{S}' = \emptyset$. Therefore, every state reached after $\delta_r + T_r + T_\alpha$ will be admissible\footnote{This proof is adopted from work~\cite{rt-reach}.}.
\end{proof}


As a direct result of this theorem, after each restart the safety controller remains in charge until a $\delta_r$ is found that satisfies the above conditions. Algorithm~\ref{alg:find_restart_time} shows the pseudo-code of system operation. 
Lines~\ref{line:startoffind} to~\ref{line:endoffind} represent the $\texttt{FindRestartTime}(x)$ function which uses the conditions of Theorem~\ref{thm:safety} to find a safe restart time. 


\begin{algorithm}[ht]
	
	\newcommand{\algorithmicbreak}{\textbf{break}}
	\newcommand{\BREAK}{\STATE \algorithmicbreak}
	\renewcommand\algorithmiccomment[1]{%
		{\it /* {#1} */} %
	}
	\renewcommand{\algorithmicrequire}{\textbf{Input:}}
	\renewcommand{\algorithmicensure}{\textbf{Output:}}
	
	\begin{algorithmic}[1]
		\begin{footnotesize}
%			\REQUIRE $x$: most recent state of the system
%			\ENSURE \texttt{bool} $\mathtt{timeFound}$: True if a restart time is found that satisfies the conditions of Theorem~\ref{thm:safety}, \texttt{double} $\delta_{\text{safe}}$: the restart time
			\STATE Start SC. ~~\COMMENT{SEI begins}\label{line:begin}
			\STATE %\texttt{bool}
            $\mathtt{timeFound} := $  \textbf{False} 
			\WHILE{$\mathtt{timeFound} ==$ \textbf{False}}
			
			\STATE $x:=$ most recent state of the system from Sensors \label{line:startoffind}

			\STATE %\texttt{double} 
  $\mathtt{\delta_{\text{candidate}}} := \delta_{\text{init}}$ ~~\COMMENT{initialize the restart time}

			\STATE $\mathtt{startTime}$ = currentTime()
			\WHILE{currentTime() - $\mathtt{startTime}$ \textless $T_s$}
			\IF {conditions of Theorem~\ref{thm:safety} are true for $\delta_{\text{candidate}}$} \label{line:thm}
			\STATE $\delta_{\text{safe}} := \delta_{\text{candidate}}$
			\STATE $\delta_{\text{candidate}}:= \delta_{\text{candidate}} + \mathsf{INC\_STEP}$ ~\COMMENT{increase the $\delta_{\text{candidate}}$}
			\ELSE 
			\STATE $\delta_{\text{candidate}}:= \delta_{\text{candidate}} - \mathsf{INC\_STEP}$
			~\COMMENT{decrease the $\delta_{\text{candidate}}$}
			\ENDIF
			\ENDWHILE		\label{line:endoffind}	
			
			\IF{$\delta_{\text{safe}} >$ currentTime() - startTime} \label{line:elapsedTimeStart}
			\STATE$\delta_{\text{safe}} = \delta_{\text{safe}} - $(startTime = currentTime())			
			\STATE $\mathtt{timeFound} := $ \textbf{True}			
			\ENDIF \label{line:elapsedTimeEnd}

			
			\ENDWHILE
			\STATE Send $\delta_{\text{safe}}$ to RoT. ~~\COMMENT{Set the next restart time.}	
			
			\STATE Activate external interfaces.~~\COMMENT{SEI ends.}
			\STATE Terminate SC and start the main controller.
			
			\STATE When RoT sends the restart signal to hardware restart pin:
            \STATE \hspace*{1em} Restart the system 
            \STATE \hspace*{1em} Repeats the procedure from beginning (\eg from Line~\ref{line:begin})
			
%			\RETURN  $\mathtt{timeFound}$ %, $\delta_\text{safe}$
			
		\end{footnotesize}
		
	\end{algorithmic}
	\caption{Pseudo-code of system operation}
	\label{alg:find_restart_time}
\end{algorithm}


%
%\begin{algorithm}[ht]
%	
%	\newcommand{\algorithmicbreak}{\textbf{break}}
%	\newcommand{\BREAK}{\STATE \algorithmicbreak}
%	\renewcommand\algorithmiccomment[1]{%
%		{\it /* {#1} */} %
%	}
%	\renewcommand{\algorithmicrequire}{\textbf{Input:}}
%	\renewcommand{\algorithmicensure}{\textbf{Output:}}
%	
%	\begin{algorithmic}[1]
%		\begin{footnotesize}
%			\REQUIRE $x$: most recent state of the system
%			\ENSURE \texttt{bool} $\mathtt{timeFound}$: True if a restart time is found that satisfies the conditions of Theorem~\ref{thm:safety}, \texttt{double} $\delta_{\text{safe}}$: the restart time
%			
%			\STATE \texttt{bool} $\mathtt{\delta_{\text{candidate}}} := \delta_{init}$ ~~\COMMENT{initialize the restart time}
%			\STATE \texttt{double} $\mathtt{timeFound} := $ \textbf{False}
%			\STATE startTime = currentTime
%			\WHILE{currentTime - startTime $ \textless T_s$}
%			\IF {conditions of Theorem~\ref{thm:safety} are true for $\delta_{\text{candidate}}$}
%			\STATE $\mathtt{timeFound} := $ \textbf{True}
%			\STATE $\delta_{\text{safe}} := \delta_{\text{candidate}}$
%			\STATE $\delta_{\text{candidate}}:= \delta_{\text{candidate}} + \mathsf{INC\_STEP}$ ~\COMMENT{increase the $\delta_{\text{candidate}}$}
%			\ELSE 
%			\STATE $\delta_{\text{candidate}}:= \delta_{\text{candidate}} - \mathsf{INC\_STEP}$
%            ~\COMMENT{decrease the $\delta_{\text{candidate}}$}
%			\ENDIF
%			\ENDWHILE
%			
%			\RETURN  $\mathtt{timeFound}$, $\delta_\text{safe}$
%			
%		\end{footnotesize}
%		
%	\end{algorithmic}
%	\caption{Pseudo-code of \texttt{FindRestartTime}(x)}
%	\label{alg:find_restart_time}
%\end{algorithm}



Note that the computation time of each round of \texttt{FindRestartTime} task (Lines~\ref{line:startoffind} to~\ref{line:endoffind}) is capped by $T_s$ so that it samples the state frequently enough. In addition, evaluation of the conditions of Theorem~\ref{thm:safety} in Line~\ref{line:thm} requires finite time and is not instantaneous. To adjust for it, the elapsed time is deducted from the computed time~(Lines~\ref{line:elapsedTimeStart} to~\ref{line:elapsedTimeEnd}) when the restart time is being set in RoT. 


It is worth mentioning that in this work, the run-time computation of reachable states~(\ie $\mathsf{Reach}$ function) that is used in evaluation of the Theorem~\ref{thm:safety} conditions, is performed using the real-time reachability technique that is proposed earlier~\cite{rt-reach}. This approach uses the model of the system dynamics~(linear or non-linear) to compute reachability. Since the real actions of the adversary at run-time are unknown reachability of the system under \emph{all} possible control values is calculated (compute reachability under $UC$). As a result, the reachable set under $UC$ is the largest set of states that might be reached from the given initial state, \textit{within the specified time}.

%\subsubsection{Definitions}
%
%Before explaining the procedure, some notations and
%definitions are necessary. Note that from the definition of $\mathcal{S}$, $\mathcal{S}$ is a convex polyhedron because
%it is the intersection of a finite number of half-spaces. For a real vector $c$
%and a real number $d$, a linear inequality $c^T x \le d$ is called valid for
%$\mathcal{S}$ if  $c^T x \le d$ holds for all $x \in \mathcal{S}$. A subset $f$
%of a polyhedron $\mathcal{S}$ is called a \emph{face} of $\mathcal{S}$ if
%there exists a valid inequality $c^T x\le d$  for $\mathcal{S}$,
%so that $f$ is represented as $f = \mathcal{S} \cap \{ x: c^Tx = d \}$. 
%
%For a given face $f$, let its surface normal be $\vec{n}$. The outward direction
%normal will be either $\vec{n}$ or $-\vec{n}$. To determine which, let $v$ be a
%point such that $v\in \mathcal{S}$ and $v \not \in f$ and let one of the
%vertices of the face $f$ be $p$. Now, consider the two vectors $\vec{n}$ and
%$\vec{pv}=v-p$. If $\vec{n}\cdot\vec{pv}$ is negative, then $\vec{n}$ is facing
%outwards or vice versa. 
%
%
%Let us assume that the set of faces of the safety region is $\mathcal{F}_\mathcal{S} = \{f_1,\dots,f_n\}$. For a face $f_i$, there exists a linear inequality $c_i^Tx \leq d_i$ that is valid for $\mathcal{S}$ and we have $f_i = \mathcal{S} \cap \{ x: c_i^Tx = d_i \}$. For each face $f_i$, $m_i-1$ equidistant planes parallel to $f_i$ divide the region $\mathcal{S}$ into $m_i$ subregions  $\mathcal{R}_i = \{\rho^i_1,\dots,\rho^i_{m_i}\}$.
%Each subregion can be represented in the following form
%\begin{equation}
%\rho^i_j = \mathcal{S} \cap \{x: c_i^Tx \geq d_i - j\cdot l_i \text{ and } c_i^Tx < d_i+(j-1)l_i\}
%\end{equation}
%and, the following condition needs to hold true
%\begin{equation}
%\mathcal{S} \cap \{x: c_i^Tx = d_i - m_i\cdot l_i \} = \emptyset
%\end{equation}
%
%Length of a subregion $\rho^i_j$ in the direction of $\vec{n_i}$ can be defined as the longest vector parallel to $\vec{n_i}$ such that its start and end points are inside $\rho^i_j$. All the regions associated with with a face have equal length of $l_i$ in the direction of $\vec{n}_i$.
%
%
%\subsubsection{Computing UpperBound of Restart Time}
%
%We define $\tau_{i,j}$ as the minimum time required to reach any point on face $f_i$ from any state in $\rho^i_j$. Furthermore, we define $d^i_j$ as the maximum value of the derivative in the direction of $\vec{n_i}$ inside region $\rho^i_j$. 
%Assuming the dynamics of the system is defined using $\dot{x} = A(x,u)$, we can write
%\begin{equation}
%d_{i,j} = max\{||\langle A(x,u),\vec{n}_i \rangle|| \mid x \in \alpha^i_j, u \in \mathbb{U}\}
%\end{equation}
%where $\langle \cdot , \cdot \rangle$ represents the inner product of two vectors and $\mathbb{U}$ is the set of all possible actuation command in the physical system. For a given state $x$ in region $\rho_j^i$, $\tau_{i,j}$ can be computed using 
%\begin{equation}
%\tau_{i,j} = \sum_{k \in [1,j]} \frac{l_{i}}{d_{i,k}}
%\label{eq:regionmintime}
%\end{equation}
%
%In order to find the smallest time in which the physical system might be able to reach to the closest boundary of the safety region, we need to calculate the $\tau_{i,j}$ for all the faces and choose the smallest value. In other words, 
%\begin{equation}
%\tau_u = \min_{i \in [1,n]}\{\tau_{i,j}:  j \text{ such that }x \in \rho^i_j\}
%\label{eq:mintau}
%\end{equation}
%
%
%The value of $\tau_u$ needs to be computed after every restart, during the secure execution interval. Due to time and resource constraints, we need a mechanism to calculate $\tau_u$ in the fastest possible way.  Notice that values of $\tau_{i,j}$ for each region and each face can be computed offline for all the region and stored in the secure memory (or a different write-protected memory). However, to calculate the results for Equation~\ref{eq:mintau}, first, the region with regards to each face need to be calculated. Given state $x$, the region of the system with regards to the face $f_{i}$ is $\alpha_{i,k_i}$ where $k_i$ is 
%\begin{equation}
%k_i = \bigg\lceil \frac{\langle x-p_{i}, \vec{n}_i \rangle}{l_i}\bigg\rceil
%\label{eq:regionnumber}
%\end{equation}
%where $p_{i}$ is a point on the face $f_i$. To evaluate the Function \ref{eq:regionnumber}, the values of $p_i$, $\vec{n_i}$, and $l_i$ need to be retrieved first. In addition, to retrieve the precomputed $\tau_{i,j}$ from memory as will be shown in the rest of this section, the value of $m_i$ also needs to be stored for each face. $m_i$ is the number of regions for each face $f_i$. Hence, we propose the following memory structure for storing and retrieving all the parameters and precomputed results.
%
%$p_i$ and $\vec{n_i}$ are vectors with length equal to the number of dimensions of the system $N$. $l_i$ and $k_i$ are single values. Hence, for each face, we need $2N + 2$ memory locations to store $p_i$, $\vec{n_i}$, $k_i$, and $l_i$. Therefore, for a system with $n$ faces of safety region $\mathcal{S}$, we need $n(2N+2)$ locations in memory for parameters. After the parameters, precomputed value of each $\tau_{i,j}$ will be stored in memory address \begin{equation}
%address(\tau_{i,j}) = n(2N+2) + \sum_{k=1}^{i} (k-1) m_{k-1} + j
%\label{eq:memAddress}
%\end{equation}
%
%
%\begin{enumerate}
%	\item Retrieve $p_i$, $\vec{n_i}$, $l_i$, and $k_i$ from memory.
%	\item Compute $k_i$ for each face $f_i$ using the retrieved parameters and Equation~\ref{eq:regionnumber}.
%	\item Calculate the memory location of each $\tau_{i,k_i}$ using Equation~\ref{eq:memAddress} and retrieve them from memory
%	\item Compute $\tau_u$ using Equation~\ref{eq:mintau}
%\end{enumerate}
%
%
%
%




%
%\subsubsection{KASLR}
%I found the following text in this link: 
%http://security.stackexchange.com/questions/69054/does-kaslr-really-provide-more-security-against-exploits
%
%"Address Space Layout Randomisation was originally applied to complicate exploits, as we all know, by randomising the position of a lot of pointers on the stack. Defeating ASLR requires either of:
%
%a. bruteforcing until you accidentally find the correct random address (which requires re-launching the app and barely ever applies to KASLR)
%b. retrieving pointers that leak information about the memory layout
%
%The second option is very promising for kernels: they can't have too much of a large random offset because some hardware configurations might have a limited address space, and \textbf{most importantly kernels can't change their offset throughout their entire life cycle! This means a single memory layout leak will defeat KASLR until the machine is rebooted}. It turns out that this kind of bug is said to happen pretty often by Spender.
%
%This is exactly why Linux KASLR is weak, and even "a failure" according to Spender. The mechanism was not intended for kernels. Do read his article if you want more details. He does speak about other implementations and you should understand from the points made above that it is not the implementations only that are weak, but rather the design. KASLR needs a lot more care in how it is implemented than traditional ASLR because the conditions for exploitation are much more favourable."
%
%From another source I found this:
%
%http://forums.grsecurity.net/viewtopic.php?f=7\&t=3367
%
%"first of all, the name itself is a bit unfortunate since what is being randomized is not exactly what happens in userland. For one, userland ASLR leaves no stone unturned so to speak. That is, a proper ASLR implementation would randomize all memory areas and would do so for every new process differently. There is no equivalent of this mechanism for a kernel since once booted, the kernel image does not change its location in memory nor is it practically feasible to re-randomize it on every syscall or some other more coarse-grained boundary. In other words, it's as if in userland we applied ASLR to a single process and kept running it indefinitely in the hope that nothing bad would happen to it. At this rate we could call the long existing relocatable kernel feature in Linux KASLR as well since it's trivial to specify a new randomly chosen load address at boot time there.
%
%Second, the amount of randomization that can be applied to the base address of the kernel image is rather small due to address space size and memory management hardware constraints, a good userland ASLR implementation provides at least twice the entropy of what we can see in KASLR implementations. To balance this deficiency there's usually already some form of inadvertent brute force prevention present in that most kernels usually don't recover from the side effects of failed exploit attempts (Linux and its oops mechanisms being an exception here)."







==> for arXiv/Sections/nonphysical.tex <==
\section{Security Improvement By Restarting on Fixed Periods}
\label{sec:probability}

The approach discussed thus far, aims to achieve a very strong goal for the safety and security of CPS. However, trying to reach such strong protection guarantees for systems with fast-moving dynamics or narrow security margin~(\eg UAVs and power grid components), may result in very short restart times. Because, such systems can quickly become unstable. With such short restart times, actions such as establishing Internet-based communication, authenticating with a remote server, or performing computationally heavy tasks may become infeasible. In this section, our goal is to demonstrate that restarting the system, even when the restart time is not strictly calculated using the approach of Section~\ref{sec:securetime}, may improve the security for many systems. 

Assume $\mathcal{P}(t)$ is the \emph{probability of successful damage} that answers to the following question: "What is the probability that an attacker succeeds in damaging the system within certain $t$ time units?". In this context, \emph{damaging the system} refer to the act of forcing the plant to reach a state in the inadmissible region. Here, $t=0$ is the start of system operation from a functional state. The \emph{expected time of damage} is $E^{\mathcal{P}}(t_{\text{attack}}) = \int_0^\infty \tau \mathcal{P}(\tau).d\tau$. A countermeasure is assumed to \emph{improve the security} of the system if $E^{\hat{\mathcal{P}}}(t_{\text{attack}}) < E^{\mathcal{P}}(t_{\text{attack}})$ where $\hat{\mathcal{P}}(t)$ and $\mathcal{P}(t)$ are the probability of successful damage with and without that countermeasure in place. In the rest of this section, we will provide an intuitive discussion of the types of systems for which periodic restarting of the system improves the security \ie reduces the expected time of attack.


 

To proceed with the discussion, we assume that $\mathcal{F}(t)$ is the probability density function~(PDF) of the successful attack on the system whose value at any given time represents the relative likelihood of an attacker being able to cause damage to the physical system. The relationship between the probability of a successful attack and its PDF is  $\mathcal{P}(t) = \int_0^{t}\mathcal{F}(\tau)\cdot d\tau$.  Further, let us assume that $\hat{\mathcal{F}}(t)$ is the PDF of a successful attack on the same system when it is restarted periodically every $\delta_r$ times.
%For simplicity, we first assume that after each restart, the attacker loses all the leverage and knowledge of the system. In other words, the chances of launching at attack after each restart is the same as previous restarts. We will correct this assumption later and take the effect of gained knowledge into effect. Under this assumption, the attacker has no advantage when trying to launch attack after 1000th system restart compared to immediately after the first system boot. 
We have the following: 
\begin{equation}
\hat{\mathcal{F}}(t) = (1-\hat{\mathcal{P}}(k\delta_r))\mathcal{F}(t-k\delta_r)
\label{eq:resetPDF}
\end{equation}
where $k = \lfloor t/\delta_r \rfloor$. The term $(1-\hat{\mathcal{P}}(k\delta_r))$ is the probability of an attack not taking place in the previous $k$ restart cycles and, $\mathcal{F}(t-k\delta_r)$ is the first $\delta_r$ time units of function $\mathcal{F}$. Integrating over Equation~\ref{eq:resetPDF} results in Equation~\ref{eq:resetProb} for the probability of successful attacks with the restart-based protection.
\begin{equation}
\hat{\mathcal{P}}(t) = \hat{\mathcal{P}}(k\delta_r) + (1-\hat{\mathcal{P}}(k\delta_r))\mathcal{P}(t-k\delta_r)
\label{eq:resetProb}
\end{equation}

From equations~\ref{eq:resetPDF} and~\ref{eq:resetProb}, we can see that  $\hat{\mathcal{F}}$ and $\hat{\mathcal{P}}(t)$  are only a function of the values of $\mathcal{F}$~( and consequently $\mathcal{P}$) within the first $\delta_r$ time units.  The effectiveness of the restart-based approach on reducing probability of damage $\hat{\mathcal{P}}$ depends on two main factors: (1) distribution of probability density of the $\mathcal{F}$ within the starting $\delta_r$ segment. In other words, smaller density of $\mathcal{F}$ within the first $\delta_r$ time units leads to a smaller growth rate of $\hat{\mathcal{P}}$ which eventually results in a smaller $E^{\hat{\mathcal{P}}}(t_{\text{attack}})$. And, (2) the second factor is the growth rate of the original $\mathcal{P}$ in the time $t > \delta_r$~(\ie how does the probability of the attack without restarts is divided over time). 

We further clarify this analysis with the use of four illustrative systems in the following. Figure~\ref{fig:fig11} depicts the PDF~($\mathcal{F}$, blue line) and probability of damage function~($\mathcal{P}$, yellow line) for a demonstrative system. It also depicts the new damage PDF~($\hat{\mathcal{F}}$, red line) and probability of damage function~($\hat{\mathcal{P}}$, purple line) after the periodic restarts with a period of $20$ time units is performed on the system. Notice that, restarting reduces the probability of damage over the time for this system~($\hat{\mathcal{P}} < \mathcal{P}$). Figure~\ref{fig:fig12} depicts the same functions for a different system where the original PDF has a smaller density within the first $20$ time units~($\mu$ of the normal function in Figure~\ref{fig:fig12} is larger than Figure~\ref{fig:fig11}). As a result of this difference, $\hat{\mathcal{F}}$ is overall smaller in Figure~\ref{fig:fig12} which reduces the growth rate of $\hat{\mathcal{P}}$ in Figure~\ref{fig:fig12} compared to~\ref{fig:fig11}. This example illustrates that periodic restart-based protection is more effective on the systems where the probability of attack/damage is low within the first $\delta_r$ times of the operation.

 
\begin{figure}[h]
	\begin{center}
		\centering 
		\subfigure[$\mathcal{F}$ is a normal function with $\mu = 30$ time units $\delta = 40$. ]{\label{fig:fig11}\includegraphics[width=0.45\textwidth]{resetpdf2}}
		\subfigure[$\mathcal{F}$ is a normal function with $\mu = 80$ time units and $\delta = 40$.]		{\label{fig:fig12}\includegraphics[width=0.45\textwidth]{resetpdf1}}
		\caption{In both figures, restart time is $20$ time units. Restart-based protection results in a smaller $\hat{\mathcal{P}}$ in the system of Figure~\ref{fig:fig12}~(the purple line) because of the smaller density of function $\mathcal{F}$ within the first $20$ time units.}
		\label{fig:resetPDF1}
	\end{center}
\end{figure}


Figures~\ref{fig:fig21} and~\ref{fig:fig22} illustrate the $\mathcal{F}$,$\mathcal{P}$, $\hat{\mathcal{F}}$, and $\hat{\mathcal{P}}$ functions for two systems where $\mathcal{F}$ has the exact same values over the first $20$ time units in both systems. Notice that, the damage probability function with restarting~($\hat{\mathcal{P}}$) is the same in both systems. However, for the system of Figure~\ref{fig:fig21}, the second major attack probability occurs later than the system of Figure~\ref{fig:fig22}. As seen in \ref{fig:fig21}, function $\hat{\mathcal{P}}$ has larger values than $\mathcal{P}$ in the range of 100 to 380 time units. This example illustrates a system where periodic restart-based approach does not improve the security of the system. 

\begin{figure}[h]
	\begin{center}
		\centering 
		\subfigure[$\mathcal{F}$ consists of two normal functions with mean at  $30s$ and $350s$ and a standard deviation of 40. ]{\label{fig:fig21}\includegraphics[width=0.45\textwidth]{resetpdf3}}
		\subfigure[$\mathcal{F}$ consists of two normal functions with mean at  $30s$ and $150s$ and a standard deviation of 40.]		{\label{fig:fig22}\includegraphics[width=0.45\textwidth]{resetpdf4}}
		\caption{In both figures, restart time is $20s$ and the density of $\mathcal{F}$ within the first 20 seconds is very similar. Restart based protection is more effective in reducing $\hat{\mathcal{P}}$ in the system of Figure~\ref{fig:fig22}~(the purple line).}
		\label{fig:resetPDF2}
	\end{center}
\end{figure}

In summary, equations~\ref{eq:resetPDF} and~\ref{eq:resetProb} provide an analytical framework for system designers to utilize $\mathcal{F}$ and $\mathcal{P}$ functions~(that are properties of the particular system) and evaluate the effectiveness of restart-based protection for the target systems.  Notice that, there is an extensive body of work in the literature that studied  probabilistic risk assessment of security threats for various domains and platforms~\eg \cite{schneier1999attack,Arnold2014,kumar2015time,5399279} . Those results can be utilized to construct $\mathcal{F}$ and $\mathcal{P}$ functions for the target systems. 



%
%In a real-world scenario, over the time the attacker is able to obtain knowledge about the operation and vulnerabilities of the system and may utilize it in the future attack attempts. In order to reflect this effect in the computation of $\hat{\mathcal{P}}$, we utilize the following
%\begin{equation}
%\hat{\mathcal{P}}(t) = (1-s_k)\left(\mathcal{P}(t-k\delta_r) + \frac{k}{(k+\alpha)}(\frac{1}{\delta_r} - \mathcal{P}(t-k\delta_r))\right)
%\label{eq:resetPDFWithKnow}
%\end{equation}
%
%Here, $k = \lfloor t/\delta_r \rfloor$ and $\alpha$ is the parameter that determines the increase in the probability of the attack from each restart to the next one as a result of increased knowledge of the attacker. 
%
%In this setup, $\alpha = \infty$ indicates no knowledge gain over the consecutive restarts. Setting $\alpha = \infty$ in Equation~\ref{eq:resetPDFWithKnow} results in Equation~\ref{eq:resetPDF}. Whereas, $\alpha = 0^+$ (\ie smallest real number above 0) means that the attacker obtains complete knowledge of all the vulnerabilities and operation of the system only after one restart. In Figure~\ref{fig:resetPDFalpha}, probability function of attacks with restarting procedure $\hat{\mathcal{C}}$ under three values of $0^+$, $100$, and $\infty$ for $\alpha$ for the same system as Figure~\ref{fig:resetPDF1} is depicted. 
%
%
%\begin{figure}[ht]
%	\begin{center}
%		\includegraphics[width=0.49\textwidth]{resetPDFalpha}
%		\caption{The logical view of the proposed design.}
%		\label{fig:resetPDFalpha}
%	\end{center}
%\end{figure}
%
%\begin{theorem}
%For a given system, if $\hat{\mathcal{C}}_\infty(t) \leq \mathcal{C}(t)$ for $t\geq0$, then the smallest possible value of $\alpha$ that results in the largest knowledge transfer rate between consecutive restarts is $\alpha_{min}$ such that $\hat{\mathcal{C}}_{\alpha_{min}}(t) \leq \mathcal{C}(t)$ for $t\geq 0$.
%\label{thm:thm2}
%\end{theorem}
%
%%\begin{proof}
%	
%For any given system, the maximum possible information gain for the attacker occurs when there is no restarts that interrupt the attack attempts or to cause information loss for the attacker. In other words, in the presence of restarts, attacker only may lose information but it can never learn  more than the case where there is no restarts. 
%
%Using this basic principle, we prove this using contradiction. Let us assume that the knowledge transfer rate of the system is $\bar{\alpha}$ such that $\bar{\alpha} < \alpha_{min}$ and results in at least one $t_o$ for which $\hat{\mathcal{C}}_{\alpha_{min}}(t_0) > \mathcal{C}(t_0)$. Without the knowledge transfer we would have had $\hat{\mathcal{C}}_{\infty}(t_0) \leq \mathcal{C}(t_0)$. Hence, the increase in the probability of attacks is solely due to the accumulated knowledge of the attacker about the system up to time $t_0$. This indicates that the attacker has obtained more knowledge when the system restarts periodically than the case where there are no restarts. This is a contrast with the initial principal of the system. Hence, $\alpha_{min}$ is the smallest possible value of $\alpha$ and for all $\alpha > \alpha_{min}$ we have $\hat{\mathcal{C}}_{\alpha}(t) < \hat{\mathcal{C}}_{\alpha_{min}}(t) \leq \mathcal{C}(t)$.
%%\end{proof}
%
%Theorem~\ref{thm:thm2} indicates that even with the increased knowledge of the attacker about the system and its vulnerabilities, restarting the system reduces the probability of the system getting attacked and damaged at any given time.





==> for arXiv/Sections/related.tex <==
\section{Related Work}
\label{sec:related}

%\subsection{Security Through Randomization}
%We should review a set of randomization works.


%\subsection{Security Through Restarting}
%We should search for related work in this topic.


% \todo[inline]{
	
% 	The idea of restarting the embedded system is explored in earlier research for fault-tolerance~\cite{abdi2017application} and fault-recovery~\cite{fardin2016reset}. However, to the best of our knowledge, this paper is the first comprehensive work to utilize concept of restart to provide security.}


 



%, they can also be used to perform safe restarting to improve security. 

%
%\subsection{Restarting Using a Back Up Controller}
%
%The architecture proposed in~\cite{fardin2016reset}, is a variation of Simplex Architecture~\cite{sha1998dependable, Sha01usingsimplicity, sha1996evolving}. This design consists of two control units. First, a main control unit, also known as Complex Control unit, that may contain logical or implementation bugs. Second, a second back up controller unit called safety unit which contains a safety controller and a decision module. Components of the safety unit are logically correct and verified~(bug-free). The safety controller is able to recover and stabilize the system as long as the state is inside a recovery region. Hence, in runtime, if the state of the system is close to the boundary of the recovery region, the decision module switches the control the safety controller. As a result, misbehaviors in the complex unit~(OS or applications) does not affect the safety of the physical system.
%
%
%\begin{figure}[ht]
% \begin{center}
%   \includegraphics[width=0.49\textwidth]{architecture-resecure}
%   \caption{Logical view of Simplex architecture using extra hardware.}
%   \label{fig::simplex}
% \end{center}
%\end{figure}


%A recent work in~\cite{abdi2017application} 



%Having only Base Controller, allows the system to remain safe and tolerate software faults and recover from them~(by performing  a restart). However, the system does not make any progress towards its mission goal. To address this issue, Base Controller is complemented with a Mission controller and a Decision Module. MC is a high-performance, complex controller that drives the system towards the mission set-points. To maximize the progress towards the mission goals, in every control cycle, Decision Module checks the Mission Controller command. If it satisfies the safety requirements, it allows the Mission Controller command to be sent to the actuators. Otherwise, Base Controller command is applied to the system. By doing so, Mission Controller drives the system for as long as possible, And, whenever it is not possible, Base Controller takes the control. 



%\subsection{Restarting for Non-Safety Critical Systems}
%The idea of restarting has been used in for non-safety critical systems.

The idea of restarting the entire system or its components at run-time has been explored in earlier research in two forms of \ci \emph{revival} (\ie reactively restart a failed component) and \cii \emph{rejuvenation} (\ie prophetically restart functioning components to prevent state degradation).  
Authors in literature \cite{candea2001recursive} introduce recursively restartable systems as a design paradigm for highly available systems and uses a combination of revival and rejuvenation techniques. Earlier research~\cite{Candea03crash-onlysoftware,candea2003jagr,candea2004microreboot} illustrate the concept of microreboot that consists of having fine-grain rebootable components and trying to restart them from the smallest component to the biggest one in the presence of faults. Others in literature~\cite{vaidyanathan2005comprehensive,garg1995analysis,huang1995software} focus on failure and fault modeling and trying to find an optimal rejuvenation strategy for various systems. The above cited works are proposed for traditional (\ie \textit{non safety-critical}) computing systems such as servers and switches and are not directly applicable to safety-critical CPS. However, they demonstrate that the concept of restarting the system is considered as a reliable method to recover a faulty/compromised system.



%Unlike traditional computing platform, restarting a computational unit in charge of controlling a physical system (\eg CPS) is a challenging problem. This is because the restarting mechanism must ensure that the safety-requirements of the physical system remain satisfied during the restart.


In the context of safety-critical systems, authors proposed to utilize restarting as a recovery method from SW bugs/faults for safety-critical applications using an additional HW unit as a back up controller during the restart~\cite{fardin2016reset}. Unlike ours, the architecture is only concerned with fault-tolerance and the security aspect of the safety-critical CPS was not addressed. Other work exists~\cite{abdi2017application}  where the authors propose the procedures to design a controller (referred to as \textit{base controller}) that enable the entire computing system to be safely restarted at run-time. %This controller is called \emph{base controller} and has the following property. 
Base Controller keeps the system inside a subset of safety region by updating the actuator input at least once after every system restart. 
Similar to the previous work, this work is also concerned with the fault-tolerance and cannot provide any guarantees in presence of an adversary.
%In other words, 
%After a restart, system can restart immediately after only one command is applied to the actuators. 
%During a restart, a fresh image of all the software~(middleware, RTOS, and applications) is loaded from a read-only storage which recovers the system into an operational state. %While fault-tolerance and and fault-recovery is the primary design criteria, the authors do not consider the security issues that distinguishes the proposed method from prior research.
Further work~\cite{mhasan_resecure16} leverages the idea of restarting to improve security of safety-critical real-time systems. %Unlike our work, it does not guarantee safety of the physical system. In addition, 
However, it requires an additional customized hardware unit to execute a back up controller during the restart to maintain the plant's stability. Our approach provides guaranteed safety for the plant and is implementable on single COTS embedded system.
While the idea of restarting the embedded system is explored in earlier research for fault-tolerance, to the best of our knowledge, this paper is the first comprehensive work to utilize system-wide restarts and physical dynamics of the system to provide security for safety-critical CPS.

%This approach is based on variants of Simplex \cite{Sha01usingsimplicity} architecture (\eg \textit{system-level Simplex}~\cite{bak2009system} with \textit{reset-based recovery}~\cite{fardin2016reset}) that have moved the safety subsystem and the decision module into a dedicated hardware unit. While this isolates the trusted components from the faults and misbehavior of the complex subsystem, this framework is not suitable for the systems developed using COTS due to additional hardware (\eg safety and complex controller) requirements.  In contrast, our proposed framework decouples the security requirements from safety properties and can be developed using COTS components using a single controller.

There is a considerable overlap between real-time systems and safety-critical embedded CPS. The problem of studying various There are recent works that study the problem of attack protection and detection approaches in real-time systems. Recent work \cite{slack_cornell, securecore, securecore_memory} on dual-core based hardware/software architectural frameworks aim to protect RTS against security vulnerabilities. In literature \cite{mohan_s3a} authors leverage the deterministic execution behavior of RTS and use Simplex architecture~\cite{sha2001using} to detect intrusion while guaranteeing the safety. Despite the improved security, all these techniques have false negatives and do not provide any guarantees. In contrast, our restart-based mechanism guarantees that the attacker cannot damage the physical sub-system.
 
%Another line of research exists that emphasizes the physical aspects of CPS in attack detection/protection. Authors in~\cite{Cardenas:2011:AAP:1966913.1966959}, studied the use of physical models and the run-time behavior of the physical systems for anomaly detection. Another work~\cite{6307833} investigates the problem of detection and isolation of attacks on a water distribution network using hydrodynamic models of the system.


==> for arXiv/Sections/resiliency.tex <==
\section{{\normalfont \textsf{ReSecure}} and Attack Resiliency}

\todo[inline]{TODO:MH $-->$ Need to rewrite this section -- MH}

Most of the existing security mechanisms protect the system from specific categories of attack and providing high security assurance requires a mixture of multiple mechanisms. Even then, there are always unknown vulnerabilities that can be exploited by an attacker to perform \emph{zero-day} attacks. On the other hand, patching the OS in embedded controllers and programmable logic controllers (PLCs) against (un)known bugs and vulnerabilities is very challenging. Due to the safety-critical nature of the applications in industrial controllers, any updates to the software needs to undergo extensive testing and verification before being deployed. 
% Some malware such as the Havex remote access trojan~\cite{symantec2014cyberespionage} infects the update installers. 
% Zero-day attacks can permanently cause the complex controller to malfunction until a manual action is taken and the vulnerability is fixed. 
% Similarly, it is very difficult, if not impossible, to claim that these compromises will be detected and be recovered from. 
\textsf{ReSecure} on the other hand, guarantees complete safety of physical unit along with some graceful degradation and restoration of functionality in the presence of any type of exploits.  



In the following, we review some examples of security threats that \textsf{ReSecure} can recover.

\subsubsection{Malicious Software}
Sophisticated adversaries can create malware that seeks to infect the external media used for transfers and updates. This opens the opportunities for possible exploits and may infect the system unknowingly to the human operator \cite{state_of_em_sec}. %Code injection attacks 
Some malicious code injections requires \textit{time}, \textit{resources} and sometime \textit{physical intervention} to spread through systems. For example, the Stuxnet worm \cite{stuxnet} was able to successfully subvert industrial control systems and infect PLCs. The worm was able to get in once an infected peripheral device was connected to the main system. After gaining access, the malware 
% fetched the attack code from a remote site and 
gradually inflicted damage to the physical plant by substituting legitimate actuation commands with infected ones \textit{over a period of time}. Flame~\cite{bencsath2012cousins} is another example of malware designed specifically for espionage that spreads through USB devices and local networks. 

Such malwares get into the system from removable drives that requires physical access and later slowly spread over the network by replicating themselves. In practice, however, it is unlikely that malicious entities can gain frequent physical access to the system after every reboot. 




% Depending on the frequency of restart (which can be determined by an approach similar to that discussed in Section \ref{subsec:restart_impact}), the malicious code may not get the opportunity to spread over the system even after successful intrusion and will be wiped out once the system reboots.

\subsubsection{Stealing Sensitive Information}
An adversary may want to track side-channel signals generated by the complex controller tasks with the intention of stealing sensitive information and secrets of the system. As a matter of fact, due to the \textit{deterministic schedules} of most RTS, an attacker can extract certain system information using signals such as timing parameters of the task~\cite{cy_side_channel}, thermal profiles \cite{thermal_profile_ccs}, secret keys \cite{side_channel_key} and cache access pattern~\cite{Wang:2007:NCD:1250662.1250723}. Such side channel attacks require the adversary to perform monitoring activities for a \textit{certain period of time to improve the accuracy} of the extracted information. 
% As an example, in order to extract the execution profile of the control tasks, the attacker may need to monitor for several hyperperiods to exactly pinpoint victim tasks \cite{cy_side_channel}. The proposed restart-based method can also be effective for such cases. This is because, by utilizing the concept of 
Restarting make it possible to prevent from \textit{stabilizing} the attacker task before it can extract a certain degree of \textit{useful} information.



% It is not inconceivable that the concept of randomization can be adopted to the proposed framework in order to make the system more resilient against attacks. 




% Let us consider the scenario in which the attacker task tries to extract the legitimate (\ie victim) task’s sensitive information (\eg a crypto key), say, using a cache side-channel attack \cite{last_level_cache}. One possible approach for the attacker would be filling some cache sets with carefully-structured data before the victim task executes. Then, the victim task runs a crypto algorithm with a given input that will use some of the cache sets. Later, the attacker task can read the cache sets and measure the latencies. Such timing information will provide hints about the victim’s cryptographic algorithm and thus aid the attacker to extract the crypto key. 



\subsubsection{Denial-of-Service (DoS) Attacks}
DoS attacks is a category of attacks where the attacker exhausts the resources of the system thereby preventing the access for the legitimate user. DoS attacks can occur in two forms; \ie system-level and network-level. In system-level attacks, attacker tries to exhaust
all the memory, consume all the processor utilization or fill all the disk spaces. These eventually prevent the real-time applications from functioning. The network-level DoS relies on sending an overwhelming influx of request to overflow the target's resources. Flood of TCP/SYN packets, overflowing the data buffer and reflective pings are examples of network DoS attacks. 

Restarting can always claim all the stale resources back and enable the system to continue operation. In the RTS context, in order to perform a system-level DoS attack, the attacker may need to monitor the execution profile for the tasks using, say, side-channel attacks and then override the task code with malicious DoS routines. Besides, the DoS routines also need some time to saturate the system resources. It is worth noting that combining all these steps to launch successful attacks requires \textit{considerable} time. 

With a correct estimation of the capabilities of the attacker (how much traffic they generate or at what rate they can exhaust system resources), the system designer can formulate the cost function for the attack and find an optimal restart time (refer to Appendix). Thus we assert that the restart-based method can be a potential solution to prevent (as well as recover) the system from many DoS attacks.


%What types of attacks we can prevent? Attacks that every time when we restart we reset all the attempts of the attacker up to that point. Like DoS

%What types of Attack we can Recover? What types of Attack we can Prevent (probably a sub-part part of attacks)?




==> for arXiv/Sections/statistical_analysis.tex <==
\section{Anomaly Detection using Multivariate Statistical Analysis}

\subsubsection{Building the System Profile}

Let us consider $Y^{\ell} = \lbrace y_1^\ell, y_2^\ell, \cdots, y_K^\ell \rbrace^{\mathrm{T}}$ is a vector of $K$ signals that represents the \textit{legitimate} system behavior (\eg sensor values, actuator outputs, task execution time, GPS coordinates, battery level, \etc).
Since the range of values for different signals could be different, we use Min-Max normalization technique \cite[Ch. 3]{data_mining_book} and linearly scale the range of each signal $y_j^\ell$ from $[0, 1]$ as follows:
%\begin{eqnarray}
$y_j^{\ell} = \frac{y_j^{org} - y_j^{min}}{y_j^{max} - y_j^{min}}$,
%\end{eqnarray}
where $y_j^{org}$ represents the original (\eg unscaled) value and $y_j^{max} (y_j^{min})$ denotes maximum (minimum) value of the $j$-th signal. Let us denote $Y_i^\ell$ as the $i$-th signal vector that used to generate the \textit{trace} of normal system behavior. Hence $\mathcal{Y}^\ell = \lbrace Y_1^\ell, Y_2^\ell, \cdots, Y_N^\ell \rbrace$ is the set of $N$ legitimate signals that build a training profile (\eg used as \textit{ground truth} in our verification procedure). In practice, this set of legitimate training profile can be obtained when the system is operated in controlled environment (\eg in production mode, before actual deployment). 


In this framework we propose to use Hotelling's T-square ($\rm{T}^2$ test) distance method  \cite{t2test} to detect anomalous behaviors during secure execution intervals. This multivariate statistical technique utilizes both first order (\eg mean and variance) and second order (\eg covariance matrix) statistical measures.
We use this simple statistical analysis to obtain difference between legitimate profiles and observed signals. We incorporate $\rm{T}^2$ test  because it is known to provide high accuracy \cite{ye2002multivariate,dos_multivariate_2,  dos_multivariate_1, t2_hindawi} yet low computation overhead that is particularly suitable for detecting
anomalies in the short secure execution duration.

Hotelling's $\rm{T}^2$ statistic for each legitimate training signal profile $Y_i^\ell$ is determined by the following \cite[Ch. 5]{stat_book}:
\begin{equation} \label{eq:t2_distance}
\mathbb{T}_i^\ell = \left( Y_i^\ell - \bar{Y}^\ell \right)^{\mathrm{T}} {S^\ell}^{-1} \left( Y_i^\ell - \bar{Y}^\ell \right)
\end{equation}
where $\bar{Y}^\ell = \frac{1}{N} \sum\limits_{n=1}^N Y_n^\ell$ is the mean signal vector and ${S^\ell}^{-1}$ is the $K \times K$ dimensional covariance matrix for the $N$ training profiles. Each element of $s_{i,j}^{\ell}$ in $S^\ell$ is represented by
$s_{i,j}^\ell = \frac{1}{N-1} \sum\limits_{n=1}^{N} \left( y_{i,n}^\ell - \bar{y}_i^\ell \right) \left( y_{j,n}^\ell - \bar{y}_j^\ell \right)
$ where $y_{i,j} \in \mathcal{Y}^\ell$ represents the value of $i$-th ($1 \leq i \leq K$) signal (\eg $y_i^\ell$)  for $j$-th ($1 \leq j \leq N$) trace and $\bar{y}_i^\ell$ is the mean value of signal $y_i^\ell$ over $N$ training traces. Given set of signal traces $\mathcal{Y}^\ell$ our proposed approach for generating legitimate system profile involves in the following steps:

\begin{enumerate}[\em i)]
\item Calculate the mean signal vector $\bar{Y}^\ell$, covariance matrix $S^\ell$
and obtain the $\rm{T}^2$ distance $\mathbb{T}_i^\ell$ for $\forall Y_i^\ell \in \mathcal{Y}^\ell$ using Eq. (\ref{eq:t2_distance}).
\item Calculate the mean $\mu_{\mathbb{T}}^\ell = \frac{1}{N} \sum_{n=1}^N \mathbb{T}_n^\ell$ and standard deviation $\sigma_{\mathbb{T}}^\ell = \sqrt{\frac{1}{N-1} \sum_{n=1}^N - {\left( \mathbb{T}_n^\ell -  \mu_{\mathbb{T}}^\ell \right)}^2  }$. 
\item Obtain the legitimate system profile using $\rm{T}^2$ statistics as $\mathfrak{pro}^\ell = (\bar{Y}^\ell, S^\ell \mu_{\mathbb{T}}^\ell, \sigma_{\mathbb{T}}^\ell)$.
\end{enumerate}

%the traces of signal we then calculate the mean $\mu_{\mathbb{T}}^\ell$ and standard 
%the following algorithm illustrates to generate the  


\subsubsection{Verification and Detection}

At runtime (\eg during securing execution interval) the proposed framework will perform a \textit{health check} by comparing current signal values with the stored legitimate profile $\mathfrak{pro}^\ell$. Note that the  measures of signals in a given CPS are represented by multiple random variables, and typically, the random variables representing the signals often does not follow any particular distribution. However, if the training signal vectors $(\eg  Y_i^\ell)$ are independent and the number of training samples are sufficiently large (\eg $N > 30$), according to the central limit theorem \cite[Ch. 5]{stat_book} the $\rm{T}^2$ distance follows approximately a
normal distribution regardless of the distribution of individual signals $y_i^\ell$ ($1 \leq i \leq K$) \cite{ye2002multivariate, dos_multivariate_1, dos_multivariate_2}. Since we are interested in detection deviations from legitimate profile, we select $\mu_{\mathbb{T}}^\ell \pm \lambda \sigma_{\mathbb{T}}^\ell$ 
as an anomaly detection threshold, that is, if the $\rm{T}^2$ distance for
 an observation %$i$ (referred to as $\mathbb{T}_i^o$) 
 (\ie $\mathbb{T}^o$)
 is \textit{not} within the range $[\mu_{\mathbb{T}}^\ell - \lambda \sigma_{\mathbb{T}}^\ell, \mu_{\mathbb{T}}^\ell + \lambda \sigma_{\mathbb{T}}^\ell]$ we mark the set of signals as anomaly, where $\lambda$ represents the confidence interval, usually ranging from $1$ to $3$ for confidence
levels ranging from 68\% to 99.7\% \cite{dos_multivariate_2, dos_multivariate_1}. 

Given the legitimate profile $\mathfrak{p}^\ell$, when the set of (normalized) signal vector $Y^{o} = \lbrace y_1^o, y_2^o, \cdots, y_K^o \rbrace^{\mathrm{T}}$ is accessed at the secure execution interval, we can therefore classify the signals (\eg normal or anomalous) based on the aforesaid detection threshold. The overall detection procedure is summarized in Algorithm \ref{alg:t2_int_detect}.


\begin{algorithm}[t]

\newcommand{\algorithmicbreak}{\textbf{break}}
\newcommand{\BREAK}{\STATE \algorithmicbreak}
\renewcommand\algorithmiccomment[1]{%
 {\it /* {#1} */} %
}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
    \renewcommand{\algorithmicensure}{\textbf{Output:}}

\begin{algorithmic}[1]
\begin{footnotesize}
\REQUIRE The legitimate profile $\mathfrak{pro}^\ell = (\bar{Y}^\ell, S^\ell \mu_{\mathbb{T}}^\ell, \sigma_{\mathbb{T}}^\ell)$, confidence level of detection $\lambda$ and the set of normalized observation signals $Y^{o} = \lbrace y_1^o, y_2^o, \cdots, y_K^o \rbrace^{\mathrm{T}}$
    \ENSURE The boolean variable $\mathtt{isAnomalous}$ indicates whether the observation signals $Y^{o}$ are \textit{normal} or \textit{anomalous}
\vspace{0.2em}
%\vspace*{-0.5em}

\STATE $\mathtt{isAnomalous} := \textbf{true}$ ~~\COMMENT{initialize the boolean variable}

\STATE Calculate $\rm{T}^2$ distance for observed signals as follows:
$$\mathbb{T}^o =  \left( Y^o - \bar{Y}^\ell \right)^{\mathrm{T}} {S^\ell}^{-1} \left( Y^o - \bar{Y}^\ell \right)$$


\IF {$\mathbb{T}_i^o \in [\mu_{\mathbb{T}}^\ell - \lambda \sigma_{\mathbb{T}}^\ell, \mu_{\mathbb{T}}^\ell + \lambda \sigma_{\mathbb{T}}^\ell]$}
\STATE \COMMENT{within threshold range, normal behavior}
\STATE $\mathtt{isAnomalous} := \textbf{false}$  
				\ENDIF
        
                
       \RETURN  $\mathtt{isAnomalous}$

\end{footnotesize}

\end{algorithmic}
\caption{Intrusion detection based on $\rm{T}^2$ statistics}
\label{alg:t2_int_detect}
\end{algorithm}





